Exploration Bonus for Regret Minimization in Undiscounted Discrete and Continuous Markov Decision Processes

We introduce and analyse two algorithms for exploration-exploitation in discrete and continuous Markov Decision Processes (MDPs) based on exploration bonuses. SCAL$^+$ is a variant of SCAL (Fruit et al., 2018) that performs efficient exploration-exploitation in any unknown weakly-communicating MDP for which an upper bound C on the span of the optimal bias function is known. For an MDP with $S$ states, $A$ actions and $\Gamma \leq S$ possible next states, we prove that SCAL$^+$ achieves the same theoretical guarantees as SCAL (i.e., a high probability regret bound of $\widetilde{O}(C\sqrt{\Gamma SAT})$), with a much smaller computational complexity. Similarly, C-SCAL$^+$ exploits an exploration bonus to achieve sublinear regret in any undiscounted MDP with continuous state space. We show that C-SCAL$^+$ achieves the same regret bound as UCCRL (Ortner and Ryabko, 2012) while being the first implementable algorithm with regret guarantees in this setting. While optimistic algorithms such as UCRL, SCAL or UCCRL maintain a high-confidence set of plausible MDPs around the true unknown MDP, SCAL$^+$ and C-SCAL$^+$ leverage on an exploration bonus to directly plan on the empirically estimated MDP, thus being more computationally efficient.

==> backup20180923/algo_bonus.tex <==
\begin{figure}[t]
\renewcommand\figurename{\small Figure}
\begin{minipage}{\columnwidth}
%\vspace{-0.3in}
\bookboxx{
        \textbf{Input:} Confidence $\delta \in ]0,1[$, $r_{\max}$, $\calS$ ($\mathcal{I}$ for \scalcont), $\A$, a constant $c \geq 0$

%\noindent \textbf{Initialization:} Set $i= 1$, and observe initial state $s_0$.\\

\noindent \textbf{For} episodes $k=1, 2, ...$ \textbf{do}

\begin{enumerate}[leftmargin=4mm,itemsep=0mm]
\item Set $t_k = t$ and episode counters $\nu_k (s,a) = 0$.

\item Compute estimates $\wb{p}_k(I(s') | I(s),a)$, $\wb{r}_k(I(s),a)$, $b_k(I(s),a)$ (Eq.~\ref{eq:exploration.bonus} or~\ref{eq:exploration.bonus.cont}) and build the MDP $\wh{M}_k^+$ (\bonusscal) or $\wh{M}^{ag+}_k$ (\scalcont).

\item Compute an $\rmaxbound/\sqrt{t_k}$-approximate solution of Eq.~\ref{eq:opt.superior.spanc} on $\wh{M}_k^+$ (\bonusscal) or $\wh{M}^{ag+}_k$ (\scalcont)
        %(with $\wh{M}^{ag+}_k$ instead of $\wh{M}_k^+$ for \scalcont) and the associated $\wt{\pi}_k$

%\item Use \regopt to compute an $1/\sqrt{t_k}$-approximation $\widetilde{\pi}_k$ of the solution of Eq.~\ref{eq:optimistic.policy.relaxedregalc} where $\mathcal{M}_k$ is replaced by $\mathcal{M}_k^{\ddagger}$ 
%
\item Sample action $a_t \sim \wt{\pi}_k(\cdot|I(s_t))$.

\item \textbf{While} $\nu_k(I(s_t),a_t) \leq \max\{1, N_k(I(s_t),a_t)\}$ \textbf{do}
%
\begin{enumerate}[leftmargin=4mm,itemsep=-1mm]
        \item Execute $a_t$, obtain reward $r_{t}$, and observe next state $s_{t+1}$.
        \item Set $\nu_k (s_t,a_t) \pluseq 1$.
        \item Sample action $a_{t+1} \sim \wt{\pi}_k(\cdot|I(s_{t+1}))$ and set $t \pluseq 1$.
\end{enumerate}

\item Set $N_{k+1}(s,a) = N_{k}(s,a)+ \nu_k(s,a)$.
\end{enumerate}
}
 \vspace{-0.1in}
 \caption{\small Structure of \bonusscal and \scalcont. For \bonusscal by definition we have $I(s) = s$.}
\label{fig:ucrl.constrained}
% \vspace{-0.2in}
\end{minipage}
\vspace{-0.2in}
\end{figure}




==> backup20180923/app_probability.tex <==
% !TEX root = main.tex

\section{Results of probability theory} \label{app:prob.res}

\subsection{Reminder}

We start by recalling some well-known properties of filtrations, stopping times and martingales \citep[Chapter 2]{klenke2013probability}. For simplicity, we use ``\as'' to denote ``almost surely'' (\ie~with probability 1). By default, when we don't mention the probability of an event, we mean that it has probability 1. When clear from the context, we omit to specify with respect to which probability distribution the result holds. In this section, we consider a probability space $(\Omega, \F, \Prob)$. We call \emph{filtration} any \emph{increasing} (for the inclusion) sequence of sub-\sigalgs~ of $\F$ \ie $(\F_n)_{n \in \Na}$ where $\forall n \in \Na$, $ \F_{n} \subseteq \F_{n+1} \subseteq \F$. We denote by $\F_{\infty} := \cup_{n \in \Na} \F_n$. For any sub-\sigalg~ $\G \subseteq \F$, we say that a real-valued random variable (\rv) $X : \Omega \rightarrow \Re^d$ is $\G$-measurable if for all borel sets $B \in \mathcal{B}\left(\Re^d\right)$, $X^{-1}(B) \in \G$. We say that $X$ is \emph{$\G$-integrable} if it is $\G$-measurable and $\E \big[|X |\big] < +\infty$ (componentwise). We call \emph{stochastic process} any sequence of \rv $ (X_n)_{n \in \Na}$. We say that the stochastic process $(X_n)_{n \in \Na}$ is \emph{adapted} to the filtration $(\F_n)_{n \in \Na}$ if for all $n\in \Na$, $X_n$ is $\F_n$-measurable. In this case, the sequence $(X_n, \F_n)_{n \in \Na}$ is called an \emph{adapted sequence}. If in addition, $X_n$ is integrable for all $n \in \Na$ then we say that $(X_n, \F_n)_{n \in \Na}$ is an integrable adapted sequence. We say that a stochastic process $(X_n)_{n \in \Na}$ is almost surely:
\begin{enumerate}[topsep=0pt, partopsep=0pt]
 \itemsep0em 
 \item \emph{increasing} (resp. \emph{strictly increasing}) if for all $n \geq N$, $\Prob \left( X_n \leq X_{n+1}  \right) =1$ (resp. $\Prob \left( X_n < X_{n+1}  \right) =1$),
 \item \emph{bounded} if there exists a universal constant $K$ such that for all $n \in \Na$, $\Prob \left( X_n < K \right) =1$,
 \item \emph{predictable} if $X_{n+1}$ is $\F_{n}$-measurable for all $n \in \Na$.
%  \item \emph{nilpotent} if there exists $N \in \Na$ such that for all $n \geq N$, $\Prob \left( X_n = 0 \right) =1$.
\end{enumerate}

\begin{definition}[Conditional expectation]\label{D:cond_exp}
 Let $X$ be an $\F$-integrable \rv with values in $\Re^d$. Let $\G \subseteq \F$ be a sub-\sigalg of $\F$. The \emph{conditional expectation of $X$ given $\G$} (denoted $\E \big[X \big| \G \big]$) is the (\as~unique) \rv that is $\G$-integrable and satisfies:
 \[ \forall A \in \G, ~~ \E \big[\one{A} \cdot\E \big[X \big| \G \big]\big] = E \big[\one{A} \cdot X \big] \]
\end{definition}

\begin{proposition}[Law of total expextations]\label{L:total_exp}
 Let $X$ be an $\F$-integrable \rv with values in $\Re^d$. For any sub-\sigalg~$\G \subseteq \F$, $\E \Big[\E \big[X \big| \G \big]\Big] = \E \big[X \big]$.
\end{proposition}

\begin{proposition}\label{L:factor_cond_exp}
 Let $X$ be an $\F$-integrable \rvrv and $\G \subseteq \F$ a sub-\sigalg. For any $\G$-integrable \rvrv $Y$ \st $YX$ is also integrable we have $\E \big[YX \big| \G \big] = Y \E \big[X \big| \G \big]$.
\end{proposition}

\begin{definition}[Stopping time]\label{D:stop_time}
 A random variable $\tau: \Omega \rightarrow \Na \cup \{+\infty\}$ is \emph{called stopping time} \wrt a filtration $(\F_n)_{n \in \Na}$ if for all $n \in \Na$, $\{ \tau =n \} \in \F_n$.
\end{definition}

\begin{definition}[\sigalg at stopping time]\label{D:stop_time_algebras}
 Let $\tau$ be a stopping time. An event \emph{prior to $\tau$} is any event $A \in \F_\infty$ \st $A \cap \{ \tau = n \} \in \F_n$ for all $n \in \Na$. The set of events prior to $\tau$ is a \sigalg denoted $\F_{\tau}$ and called \emph{\sigalg at time $\tau$}:
 \[ \F_{\tau} := \left\{A \in \F_{\infty}: ~ \forall n \in \Na,~A \cap \{\tau = n\} \in \F_n \right\}  \]
\end{definition}

\begin{proposition}\label{L:stop_time_algebras}
 Let $\tau_1$ and $\tau_2$ be two stopping times \wrt the same filtration $(\F_n)_{n \in \Na}$ \st $\tau_1 \leq \tau_2$ \as Then $\F_{\tau_1} \subseteq \F_{\tau_2}$.
\end{proposition}

\begin{definition}[Stopped Process]\label{D:process_stopped}
 Let $(X_n, \F_n)_{n \in \Na}$ be an adapted sequence with values in $\mathbbm{R}^d$. If $\tau$ is a stopping time \wrt the filtration $(\F_n)_{n \in \Na}$, then the \emph{process stopped at time $\tau$} (denoted by $X_\tau$) is the \rv defined as: \[\forall \omega \in \Omega, ~~ X_\tau(\omega) := \sum_{n \in \Na} X_n(\omega) \cdot \one{\tau(\omega) = n} ~~ \text{(\ie} ~ X_\infty(\omega) = 0 ~\text{by convention)} \]
\end{definition}

\begin{proposition}\label{L:process_stopped}
 $X_\tau$ --the process stopped at time $\tau$-- is $\F_{\tau}$-measurable.
\end{proposition}

% \begin{definition}[Martingale]\label{D:martingale}
%  An adapted sequence $(X_n, \F_n)_{n\in \Na}$ is a \emph{martingale} if for all $n \in \Na$, $X_n$ is $\F_n$-integrable and $\E\big[ X_{n+1} | \F_{n} \big] = X_n$ \as
% \end{definition}
% 
\begin{definition}[Martingale difference sequence]\label{D:mds}
 An adapted sequence $(X_n, \F_n)_{n\in \Na}$ is a \emph{martingale difference sequence} (MDS for short) if for all $n \in \Na$, $X_n$ is $\F_n$-integrable and $\E\big[ X_{n+1} | \F_{n} \big] = 0$ \as
\end{definition}
% 
% \begin{remark}
% If the adapted sequence $(X_n, \F_n)_{n\in \Na}$ is an MDS, then the sequence of partial sums $\left(Y_n := \sum_{i =0}^n X_i, \F_n \right)_{n \in \Na}$ is a martingale. Symmetrically, if $(Y_n, \F_n)_{n \in \Na}$ is a martingale, then the adapted sequence $(X_n, \F_n)_{n\in \Na}$ where $X_0 :=Y_0$ and $X_{n+1} := Y_{n+1} - Y_{n}$ ($\forall n\geq0$) is an MDS (hence the name martingale \emph{difference} sequence).
% \end{remark}
% \begin{definition}[Martingale transform]\label{D:martingale_transform}
%  Let $(X_n, \F_n)_{n\in \Na}$ be an integrable adapted sequence and $(C_n)_{n\in \Na}$ a bounded predictable process. The \emph{martingale transform} of $(X_n)_{n\in \Na}$ by $(C_n)_{n\in \Na}$ is the stochastic process $(M_n)_{n\in \Na}$ defined by: $M_n = \sum_{i=0}^{n} X_i C_i$ for all $n \in \Na$.
% \end{definition}
% 
% \begin{proposition}\label{L:martingale_transform}
%  If $(X_n, \F_n)_{n\in \Na}$ is an MDS and $(C_n)_{n\in \Na}$ is a bounded predictable process the \emph{martingale transform} of $(X_n)_{n\in \Na}$ by $(C_n)_{n\in \Na}$ is also a martingale or equivalently, the sequence $(C_n \cdot X_n, \F_n)_{n\in \Na}$ is an MDS.
% \end{proposition}

\begin{proposition}[Azuma's inequality]
 Let $(X_n, \F_n)_{n\in \Na}$ be an MDS such that $|X_n| \leq a$ \as for all $n \in \Na$. Then for all $\delta \in ]0,1[$, 
 \begin{align*}
 \Prob \left( \forall n \geq 1,~ \left| \sum_{i =1}^{n} X_i \right|  \leq a \sqrt{n \ln \left( \frac{2n}{\delta} \right)} \right) \geq 1 - \delta
 \end{align*}
\end{proposition}
\begin{proof}
 Azuma's inequality states that:
 \begin{align*}
 \Prob \left( \left| \sum_{i =1}^{n} X_i \right|  \leq a \sqrt{\frac{n}{2}\ln \left( \frac{2}{\delta} \right)} \right) \geq 1 - \delta
 \end{align*}
 We can then choose $\delta \leftarrow \frac{\delta}{2n^2}$ and take a union bound over all possible values of $n \geq 1$. The result follows by noting that $\sum_{n\geq 1}  \frac{\delta}{2n^2} < \delta$.
\end{proof}

\begin{proposition}[Freedman's inequality]
 Let $(X_n, \F_n)_{n\in \Na}$ be an MDS such that $|X_n| \leq a$ \as for all $n \in \Na$. Then for all $\delta \in ]0,1[$, 
 \begin{align*}
 \Prob \left( \forall n \geq 1,~ \left| \sum_{i =1}^{n} X_i \right|  \leq 2 \sqrt{ \left( \sum_{i =1}^{n} \Varcond{X_i}{\F_{i-1}} \right) \cdot\lnn{ \frac{4n}{\delta} }  } + 4 a \lnn{\frac{4n}{\delta}} \right) \geq 1 - \delta
 \end{align*}
\end{proposition}
\begin{proof}
 \citet{freedman1975} showed that when $a =1$:
 \begin{align*}
 \Prob \left( \forall n \geq 1,~ \sum_{i =1}^{n} X_i \geq \varepsilon, ~ \sum_{i =1}^{n} \Varcond{X_i}{\F_{i-1}} \leq k\right) \leq \expp{ \frac{-\varepsilon^2}{2 k + 2\varepsilon / 3} }
 \end{align*}
 Since $(-X_n, \F_n)_{n\in \Na}$ is also an MDS, the above inequality holds also in absolute value (with a factor $2$ appearing in front of the exponential term after taking a union bound). In order to reverse the inequality (\ie replace $\varepsilon$ by $\delta$), we can use the same technique as \citet[Section 2]{Cesa-Bianchi:2005}. Finally, to account for the case where $a \neq 1$ we can simply apply the result to $(X_n/a, \F_n)_{n\in \Na}$.
\end{proof}


\subsection{A useful result for the regret proof}

In this section we prove a very simple theorem that will be extensively used later to derive the regret proof. We start with useful lemmas and definitions.
% \begin{lemma}
%  Let $(X_n, \F_n)_{n\in \Na}$ be an integrable adapted sequence and $(C_n)_{n\in \Na}$ a bounded predictable process. The sequence $(Y_n, \F_n)_{n\in\Na}$ defined by $Y_0 := 0$ and for all $n \in \Na$, $Y_{n+1} :=  C_{n+1} \cdot \left(X_{n+1} - \E \big[X_{n+1} \big| \F_{n} \big] \right)$, is an MDS.
% \end{lemma}
% 
% \begin{remark}
%  See martingale transform  which is the discrete analogue of stochastic integration.
% \end{remark}
% Equivalent of previous lemma but for a sequence of stopping times:
\begin{lemma}\label{L:stop_time_algebras2}
 Let $\tau_1$ and $\tau_2$ be two stopping times \wrt the same filtration $(\F_n)_{n \in \Na}$. We say that $\tau_1 < \tau_2$ \as if $\Prob \left( \{ \tau_1 < \tau_2 \} \cup \{\tau_1 = \tau_2 = +\infty \} \right) = 1$. If $\tau_1 < \tau_2$ \as then $\F_{\tau_1 + 1} \subseteq \F_{\tau_2}$.
\end{lemma}
\begin{proof}
 If $\tau_1 < \tau_2$ then $\tau_1 +1 \leq \tau_2$ since $\tau_1$ is an integer-valued \rv If $\tau_1 = \tau_2 = +\infty$ then $\tau_1 +1 = +\infty$ and so $\tau_1 +1 = \tau_2$. In conclusion, $\tau_1 +1 \leq \tau_2$ \as and so by Prop.~\ref{L:stop_time_algebras}, $\F_{\tau_1 + 1} \subseteq \F_{\tau_2}$.
\end{proof}

\begin{definition}
 We say that a sequence of stopping times $(\tau_m)_{m \in \Na}$ \wrt $(\F_n)_{n\in \Na}$ is \emph{strictly increasing} if $\tau_m < \tau_{m+1}$ \as for all $m \geq 0$.
\end{definition}

\begin{lemma}\label{L:mds_stop_time}
 Let $(X_n, \F_n)_{n\in \Na}$ be a bounded adapted sequence, let $(\tau_m)_{m \in \Na}$ be a strictly increasing sequence of stopping times \wrt $(\F_n)_{n\in \Na}$ and let $(C_n)_{n\in \Na}$ be a bounded predictable process. For all $m \in \Na$, define $Y_{m} := C_{\tau_m+1} \cdot \left(X_{\tau_m+1} - \E \big[X_{\tau_m+1} \big| \F_{\tau_{m}} \big] \right)$ and $\G_{m} :=\F_{\tau_{m \smallplus1}} $. Then, $(Y_m,\G_m)_{m\in\Na}$ is an MDS.
\end{lemma}
\begin{proof}
 By assumption, for any $m \in \Na$, $\tau_m < \tau_{m+1}$ \as and Prop.~\ref{L:stop_time_algebras} implies that $\F_{\tau_m} \subseteq \F_{\tau_{m\smallplus 1}}$. As a consequence, $(\G_m)_{m\in \Na} = (\F_{\tau_{m\smallplus 1}})_{m\in \Na}$ is a filtration. By Prop.~\ref{L:process_stopped} we know that $X_{\tau_m +1}$ is $\F_{\tau_m +1}$-measurable and Lem.~\ref{L:stop_time_algebras2} implies that $\F_{\tau_m + 1} \subseteq \F_{\tau_{m+1}} = \G_m$ so $X_{\tau_m +1}$ is $\G_m$-measurable. Similarly, $C_{\tau_m+1}$ is $\F_{\tau_m}$-measurable and $\F_{\tau_m} \subseteq \F_{\tau_{m\smallplus 1}}$ so it is $\G_m$-measurable too. Finally, $\E \big[X_{\tau_m+1} \big| \F_{\tau_{m}} \big]$ is $\F_{\tau_m}$-measurable by definition (see Def.~\ref{D:cond_exp}). Therefore, $Y_m$ is $\G_m$-measurable.
 
 Since by assumption $X_n$ is \as bounded ($\Prob \left( X_n < K \right) =1$ for all $n\geq 0$), we can write \as (see Def.~\ref{D:process_stopped}) \[\big|X_{\tau_m +1}\big| = \left|\sum_{n=0}^{+\infty} \one{\tau_m +1 = n} \cdot X_n \right| \leq \sum_{n=0}^{+\infty} \one{\tau_m +1 = n} \cdot \left|X_n \right| \leq K \sum_{n=0}^{+\infty} \one{\tau_m +1 = n} = K\]
 Thus, $X_{\tau_m +1}$ is \as bounded hence integrable implying that $\E \big[X_{\tau_m+1} \big| \F_{\tau_m} \big]$ is well-defined (see Def.~\ref{D:cond_exp}).
 $C_n$ is also \as bounded by assumption implying that $Y_{m}$ is \as bounded and so integrable.
 
 Finally, since $C_{\tau_m+1}$ is $\F_{\tau_m}$-measurable we can apply Prop.~\ref{L:factor_cond_exp} and we obtain:
 \begin{align*}
  \E \big[Y_{m+1} \big| \G_m \big] &= C_{\tau_m+1} \cdot\E \Big[X_{\tau_m+1}  - \E \big[X_{\tau_m+1} \big| \F_{\tau_m} \big] \Big| \F_{\tau_m} \Big]\\
  &= C_{\tau_m+1} \cdot \Big(\E \big[X_{\tau_m+1} \big| \F_{\tau_m} \big] - \E \big[X_{\tau_m+1} \big| \F_{\tau_m} \big] \Big) = 0
 \end{align*} which concludes the proof.
\end{proof}

\begin{theorem}\label{T:inequality_stop_mds}
Let $(X_n, \F_n)_{n\in \Na}$ be an adapted sequence \as bounded by $a_1$, let $(\tau_m)_{m \in \Na}$ be a strictly increasing sequence of stopping times \wrt $(\F_n)_{n\in \Na}$ and let $(C_n)_{n\in \Na}$ be a predictable process \as bounded by $a_2$. If $(Y_m,\G_m)_{m\in\Na}$ is defined as in Lem.~\ref{L:mds_stop_time} then the following concentration inequalities hold:
 \begin{align*}
  &\Prob \left( \forall m \geq 1, ~ \left| \sum_{i =1}^{m} Y_m  \right|  \leq a_1 a_2\sqrt{m \ln \left( \frac{2 m }{\delta} \right)} \right) \geq 1 - \delta\\
 &\Prob \left( \forall m \geq 1,~ \left| \sum_{i =1}^{m} Y_m \right|  \leq 2 \sqrt{ \left( \sum_{i =1}^{m} \Varcond{Y_i}{\G_{i-1}} \right) \cdot\lnn{ \frac{4m}{\delta} }  } + 4 a_1 a_2 \lnn{\frac{4m}{\delta}} \right) \geq 1 - \delta
 \end{align*}
 where $\Varcond{Y_i}{\G_{i-1}} = C_{\tau_i + 1} \cdot \Varcond{X_{\tau_i +1}}{\F_{\tau_i}}$ for all $i \geq 1$.
 In particular for any $\F$-measurable integer-valued \rv $N: \Omega \rightarrow \Na$ the above inequalities hold true with $m$ replaced by $N$ \eg
  \begin{align*}
  \Prob \left(\left| \sum_{i =1}^{N} Y_m \right|  \leq a_1 a_2 \sqrt{N \ln \left( \frac{2 N }{\delta} \right)} \right) \geq 1 - \delta ~~ \dots
 \end{align*}
 
\end{theorem}
\begin{proof}
 The concentration inequalities follow from Lem.~\ref{L:mds_stop_time} and Azuma's and Freedman's inequalities. For the conditional variance, we simply notice that $C_{\tau_i + 1}$ is $\F_{\tau_i}$-measurable as shown in the proof of Lem.~\ref{L:mds_stop_time}.
If the results hold for all $n \in \Na$ and $N$ takes values in $\Na$, then the result holds for $N$ too which concludes the proof.
\end{proof}
% 
% \begin{remark}
%  Note that there are several useful special cases of Thm.~\ref{T:inequality_stop_mds} for example when the predictable process and the constant $a_2$ are simply removed from the concentration inequality (when $C_n =1$ for all $n \in \Na$ the assumptions of the theorem hold with $a_2 = 1$).
% \end{remark}

\subsection{Filtration and stopping time used in the regret proof}

For any $t \geq 0$, the \sigalg induced by the past history of state-action pairs and rewards up to time $t$ is denoted $\mathcal{F}_t:= \sigma \left( s_1, a_1, r_1, \dots, s_t, a_t \right)$ where by convention $\mathcal{F}_0 = \sigma \left( \emptyset \right)$ and $\mathcal{F}_\infty := \cup_{t\geq 0}\mathcal{F}_{t}$. 
% We also introduce a slightly different \sigalg $\mathcal{F}_t':= \sigma \left( s_1, a_1, r_1 \dots, s_t, a_t \right)$ where by convention $\mathcal{F}_0' = \sigma \left( \emptyset \right)$ and $\mathcal{F}_\infty' := \cup_{t\geq 0}\mathcal{F}_{t}'$.
Trivially, for all $t\geq 0$, $\mathcal{F}_{t} \subseteq \mathcal{F}_{t+1}$ and the filtration $\left(\mathcal{F}_t \right)_{t \geq 0}$ is denoted by $\mathbb{F}$. We recall that the sequence $(t_k)_{k \geq 1}$ (starting times of episodes $k\geq 1$) is formally defined by $t_1 :=1$ and for all $k \geq 1$, \[t_{k+1}:=1 + \inf\left\{T \geq t > t_k:~  \sum_{u=t_k}^{t -1 } \mathbbm{1}(s_u \in I(s),a_u =a) \geq \sum_{u=0}^{t_k -1 } \mathbbm{1}(s_u \in I(s) ,a_u =a)  \right\}.\]
where by convention $\inf \{ \emptyset \} := T $. It is immediate to see that for all $t\geq 0$, $\{ t_k = t \} \in \mathcal{F}_{t-1} \subseteq \mathcal{F}_t$ and so $t_k$ is a \emph{stopping time} \wrt filtration $\mathbb{F}$ (see Def.~\ref{D:stop_time}).



==> backup20180923/app_proof_regret_cont.tex <==
% !TEX root = main.tex
\subsection{Regret Proof of \scalcont (Proof of Thm.~\ref{thm:regret.scalcont})} \label{app:proof.regret.continuous} 
% We follow the proof structure of~\citep{Jaksch10,fruit2018constrained} and we use similar notation.
%
% The regret of \bonusscal after $T$ step is defined as: $\Delta(\bonusscal,T) = T g^* - \sum_{t=1}^T r_t(s_t,a_t)$.
In this section we provide a complete proof of the regret bound for \scalcont.
Defining $\Delta_k=\sum_{s \in \mathcal{S}} \nu_k(s) \left(g^* - \sum_{a \in \A_{s_t}} r(s,a)\widetilde{\pi}_{k}(s,a)\right)$ and using the arguments in~\citep{Jaksch10,fruit2018constrained}, it holds with probability at least $1-\frac{\delta}{20T^{5/4}}$ that:
%\begin{align}\label{eq:splitting}
 $\Delta(\bonusscal,T) \leq \sum_{k=1}^m \Delta_k + \rmaxbound\sqrt{\frac{5}{2}T\ln \left(\frac{11T}{\delta}\right)}$.
%\end{align}
Note that $\nu_k(s)$ is the total number of observation of state $s$ in episode $k$ and is well-defined for $s$ lying in $[0,1]$.
Finally, recall that for any subset $I\subseteq \mathcal{S}$, the sum $\sum_{s \in I} u_{s} $ is also well-defined as long as the collection $\left(u_{s} \right)_{s \in I}$ contains only a finite number of non-zero elements.

\vspace{.2cm}
\noindent \tikz{
        \node[draw=red!90!black, color=red!90!black, text width=0.985\textwidth]{\faExclamationTriangle~~~ In this section we will abuse of notation and write $p(\cdot|s,a)^\transp v = \int_\calS p(s'|s,a) v(s') \mathrm{d}s'$ for any probability density function $p$ defined on $\calS = [0,1]$.};
}


\subsubsection{Optimism and Bellman Equation}
We consider the case where $\Delta_k \cdot \one{g^*_c(\wh{M}^{ag+}_k) \geq g^*}$, the complementary case is (cumulatively) bounded by $\rmaxbound \sqrt{T}$ as in~\citep{Jaksch10,fruit2018constrained}. 
Denote by $\wt{g}_k:= 1/2(\max \{v_{n+1} - v_n\} + \min \{v_{n+1} - v_n\})$ where $v_n$ is the value function returned by \scopt{($0,\overline{s},\gamma_k,\varepsilon_k$)}. 
Remember that $v_n, v_{n+1} \in \mathbb{R}^S$ are discrete vectors obtained at different iterations of \scopt on $\wh{M}_k^{ag+}$.
The stopping condition of \scopt is such that~\citep[see][]{fruit2018constrained}
\begin{align*}
        \wt{g}_k \geq g_c^*(\wh{M}_k^{ag+}) - \underbrace{\varepsilon_k}_{=\rmaxbound /\sqrt{t_k}} \overbrace{\geq}^{\text{Lem.~\ref{L:optimism}}} g^* - \frac{\rmaxbound}{\sqrt{t_k}}
\end{align*}
implying:
\begin{align*}
        \Delta_k \cdot \one{g^*_c(\wh{M}_k^{ag+}) \geq g^*} 
\leq \rmaxbound \sum_{s \in \mathcal{S}} \frac{ \nu_k(s)}{\sqrt{t_k}} 
+ \sum_{s \in \mathcal{S}} \nu_k(s) \Bigg(
\underbrace{\wt{g}_k - \sum_{a \in\mathcal{A}_{s}} r(s,a)\widetilde{\pi}_{k}(s,a)}_{:= \Delta'_k(s)}
\Bigg)
\end{align*}
Note that we can associated a continuos piecewise-constant function to the discrete vector $v_n$: $h_n(s) = v_n(I(s)),~\forall s\in \calS$.
A consequence of Lem.~\ref{L:bonus.inequality.continuous}\emph{(b)} applied to vector $h_n$ is that $-r(s,a) \leq d_k(s,a) -\wb{r}_k(s,a) + \left( p(\cdot|s,a) -  \wh{p}_k(\cdot|s,a) \right)^\transp h_n$. Note that we cannot use the tighter version $\emph{(a)}$ since it does not hold for any function $h_n$. Moreover, by definition $\wb{r}_k(s,a) = \wb{r}_k^{ag}(I(s),a) = \wh{r}_k(s,a) - b_k(s,a)$. Therefore:
\begin{equation}
        \label{E:delta_prime}
        \begin{aligned}
        \Delta'_k(s) &\leq 
        \wt{g}_k -  \sum_{a \in \A_s} \wt{\pi}_k(s,a)\bigg( \underbrace{\wh{r}_k(s,a)}_{:= \wh{r}^{ag}_k(I(s),a)}  + \wh{p}_k(\cdot|s,a)^\transp h_n\bigg)\\
        &\quad{} + \sum_{a \in \A_s} \wt{\pi}_k(s,a) \bigg( \underbrace{b_k(s,a)}_{:= b_k(I(s),a)} + d_k(s,a) + p(\cdot|s,a) ^\transp h_n \bigg)
        \end{aligned}
\end{equation}
A direct consequence of the stopping condition used by \scopt (see Thm. 18 in~\citep{fruit2018constrained}) is that: $\forall J \in \mathcal{I}$,
\begin{equation}\label{E:gerror.app2}
%        \forall J \in \mathcal{I},~~ 
        \bigg| \wt{g}_k - \sum_{a \in \A} \sum_{i \in \{1,2\}} \wh{r}_k^{ag+}(J, a_i) \wt{\pi}_k(J,a_i) + v_n(J)
        - \sum_{a \in \A} \sum_{i \in \{1,2\}}\wt{\pi}_k(J,a_i)\wh{p}_k^{ag+}(\cdot|J,a_i)^\transp v_n \bigg| \leq \frac{\rmaxbound }{\sqrt{t_k}}
\end{equation}
Recall that by definition: $\wt{\pi}_k(J,a) = \wt{\pi}_k(J,a_1) + \wt{\pi}_k(J,a_2)$, $\wh{r}_k^{ag+}(J, a_i) \leq \wh{r}_k^{ag}(J, a)$ (since $\wh{r}_k^{ag+}(J, a_1) = \wh{r}_k^{ag}(J, a)$ and $\wh{r}_k^{ag+}(J, a_2) = 0$) and $\wh{p}_k^{ag}(\cdot|J,a) = \wh{p}_k^{ag+}(\cdot|J,a_i) $. We can thus write:
%
\begin{equation}\label{eq:mdp.augmentation.props}
\begin{aligned}
        &\sum_{a \in \A} \wh{r}_k^{ag}(J,a) \wt{\pi}_k(J,a) 
        = \sum_{a \in \A} \sum_{i \in \{1,2\}} \wh{r}_k^{ag}(J, a) \wt{\pi}_k(J,a_i)
        \geq\sum_{a \in \A} \sum_{i \in \{1,2\}} \wh{r}_k^{ag+}(J, a_i) \wt{\pi}_k(J,a_i)\\
        & \text{and} ~ \sum_{a \in \A} \wt{\pi}_k(s,a)  \wh{p}_k^{ag}(\cdot|J,a) 
        = \sum_{a \in \A} \sum_{i \in \{1,2\}} \wt{\pi}_k(J,a_i) \wh{p}_k^{ag+}(\cdot|J,a_i) 
\end{aligned}
\end{equation}
Plugging this last two equations into \eqref{E:gerror.app2} and
% \begin{equation*}
%         \begin{aligned}
%                 \forall J \in \mathcal{I}, ~~~ \wt{g}_k - \sum_{a \in \A} \wt{\pi}_k(J,a) \bigg( \wh{r}_k^{ag}(J,a)  + \wh{p}_k^{ag}(\cdot|s,a)^\transp v_n\bigg) \leq - v_n(J) + \frac{\rmaxbound }{\sqrt{t_k}}
%         \end{aligned}
% \end{equation*}
%
using Eq.~\ref{eq:piecewise_vector_proba} (\ie $\wh{p}_k(\cdot|s,a)^\transp h_n = \wh{p}^{ag}_k(\cdot|s,a)^\transp v_n$), the fact $h_n(s) = v_n(I(s))$, $\wh{r}_k(s,a) = \wh{r}^{ag}_k(I(s),a)$, and $\wt{\pi}_k(s,a) = \wt{\pi}_k(I(s),a)$, we obtain:
\begin{equation}\label{E:gerror.app}
        \begin{aligned}
                \forall s \in \calS, ~~~ \wt{g}_k - \sum_{a \in \A} \wt{\pi}_k(s,a) \bigg( \wh{r}_k(s,a)  + \wh{p}_k(\cdot|s,a)^\transp h_n\bigg) \leq - h_n(s) + \frac{\rmaxbound }{\sqrt{t_k}}
\end{aligned}
\end{equation}
%
Combining \eqref{E:gerror.app} with \eqref{E:delta_prime} we have:
\begin{align*}
        \Delta'_k(s) \leq \sum_{a\in\A_s} \wt{\pi}_k(s,a) \bigg( d_k(s,a) + \underbrace{b_k(s,a)}_{\leq d_k(s,a)} + p(\cdot|s,a)^\transp h_n \bigg) - h_n(s) + \frac{\rmaxbound }{\sqrt{t_k}}\\
\end{align*}
%
Note that $d_k(s,a) \geq b_k(s,a)$ for any $(s,a) \in \calS \times \A$ since the term $\phi_{p,k}^{sa}$ contains a $\sqrt{S}$ dependence that is not present in $\beta_{p,k}^{sa}$.
Since the dominant term is given by $d_k(s,a)$, we will consider the following loser upper-bound $d_k(s,a) + b_k(s,a) \leq 2 d_k(s,a)$ in the remaining of the proof.
%
We can now state that
\begin{equation}
        \label{eq:deltak.bound}
\begin{aligned}
        \Delta_k &\leq  \underbrace{\sum_s \nu_k(s) \left( \sum_a \left( \wt{\pi}_k(s,a) p(\cdot|s,a)^\transp w_k \right) - w_k(s) \right)}_{\xi_k}\\
                 &\quad{} + 2 \sum_{s,a} \nu_k(s) \wt{\pi}_k(s,a)  d_k(s,a) + 2\rmaxbound \sum_{s \in \mathcal{S}} \frac{ \nu_k(s)}{\sqrt{t_k}}
\end{aligned}
\end{equation}
where $w_k$ is obtained by ``recentering'' $h_n$ around $0$ so that $\|w_k\|_\infty = \SP{w_k}/2 \leq c/2$~\citep[see][App. F4]{fruit2018constrained}.
Then, similarly to what is done in~\citep[][Sec. 4.3.2]{Jaksch10} and~\citep[][App. F.7, pg. 32]{fruit2018constrained}, we have
\begin{align*}
        \xi_k 
        &= \sum_{t=t_k}^{t_{k+1}-1} 
        \underbrace{\sum_a \int p(s'|s_t,a_t) \wt{\pi}_k(s_t,a_t) w_k(s') \mathrm{d}s'  - w_k(s_{t+1})}_{:=X_t} 
        +  \sum_{t=t_k}^{t_{k+1}-1} w_k(s_{t+1}) - w_k(s_t)\\
        &= \sum_{t=t_k}^{t_{k+1}-1} X_t
        +  \underbrace{w_k(s_{t_k+1}) - w_k(s_{t_k})}_{\leq \SP{w_k} \leq c}
\end{align*}
Given the filtration $\mathcal{F}_t = \sigma\left(s_1,a_1,r_1,\dots, s_{t+1} \right)$, $X_t$ is an MDS since $|X_t| \leq c$ and $\mathbb{E}[X_t|\mathcal{F}_{t-1}]=0$ since $\wt{\pi}_{k_t}$ is $\mathcal{F}_{t-1}$-measurable.
By using Azuma inequality we have that with probability at least $1 - \frac{\delta}{20 T^{5/4}}$
\begin{equation}\label{eq:pminusone.inequality}
        \sum_{k=1}^m \xi_k \leq c \sqrt{\frac{5}{2}T\ln \left(\frac{11T}{\delta}\right)} +   m c
\end{equation}
with $m \leq SA \log_2\left(\frac{8T}{SA}\right)$ when $T \geq SA$ (see App. C.2 in~\citep{Jaksch10}).

\subsubsection{Bounding the exploration bonus}
Using the same argument in App. F.6 in~\citep{fruit2018constrained} and by noticing that $d_k(s,a) \leq 2c + \rmaxbound \leq 2\max\{c, \rmaxbound\}$, we obtain with probability at least $1-\frac{\delta}{20T^{5/4}}$:
\begin{align}
        \sum_{k=1}^{m}\sum_{s,a} \nu_k(s)&\wt{\pi}_k(s,a) d_k(s,a)
        \leq \sum_{k=1}^{m}\sum_{s,a} \nu_k(s,a) d_{k}(s,a)
        + 2\max\{c,\rmaxbound\}\sqrt{\frac{5}{2}T\ln \left(\frac{11T}{\delta}\right)}
        \label{eq:bonus.mds}
\end{align}

We now gather inequalities~\eqref{eq:bonus.mds},~\eqref{eq:pminusone.inequality} and a result in~\citep[][App. F.7, pg. 33]{fruit2018constrained} into inequality~\eqref{eq:deltak.bound} summed over all the episodes $k$ which yields (after taking a union bound) that with probability at least $1 - \frac{2\delta}{20 T^{5/4}}\geq 1 - \frac{3\delta}{20 T^{5/4}}$ (for $T\geq SA$):
\begin{align}\label{eq:sum.deltak}
 \begin{split}
         \sum_{k=1}^m \Delta_k \;\mathbbm{1}\{g^*_c(\wh{M}_k) \geq g^*\} &\leq
         3\max\{c, \rmaxbound\} \sqrt{\frac{5}{2}T\ln \left(\frac{11T}{\delta}\right)}
         +  c SA\log_2\left(\frac{8T}{SA}\right)\\
 &\quad{}
 + 2\rmaxbound \left(\sqrt{2} +1 \right)\sqrt{SAT}
 + 2
        \sum_{k=1}^{m}\sum_{s,a} \nu_k(s,a) d_{k}(s,a)
 \end{split}
\end{align}
%
Let $\phi_{p,k}^{sa}$ as defined in Eq.~\ref{eq:bernstein.ci.cont}, then 
\begin{equation}\label{eq:bonus.bound.2}
\begin{aligned}
        \sum_{k=1}^{m}\sum_{s,a} \nu_k(s,a) d_{k}(s,a) 
        &\leq
        \underbrace{\sum_{k=1}^{m}\sum_{s,a} \nu_k(s,a) \beta_{r,k}^{sa}}_{\text{see p. 33~\citep{fruit2018constrained}}}
        +c \underbrace{\sum_{k=1}^m \sum_{s,a} \nu_k(s,a) \phi_{p,k}^{sa}}_{\text{see p. 33~\citep{fruit2018constrained}}}\\
        &\quad{}+ 2c \sum_{k=1}^m \sum_{s,a}\frac{\nu_k(s,a)}{N_k(s,a)+1} 
        + \underbrace{(c+\rmaxbound)}_{\leq 2\max\{c,\rmaxbound\}} L S^{-\alpha} T
\end{aligned}
\end{equation}
%
We recall that 
\begin{align*}
        \sum_{k=1}^{m}\sum_{s,a} \nu_k(s,a) \beta_{r,k}^{sa} = \wt{O}(\rmaxbound \sqrt{SAT}) ~~ \text{ and } ~~ \sum_{k=1}^m \sum_{s,a} \nu_k(s,a) \phi_{p,k}^{sa} =\wt{O}(c S\sqrt{A T} +cS^2A).
\end{align*}
%
Similarly to what done in~\citep[][Eq. 58-60]{fruit2018constrained}, we can write
\begin{equation}\label{eq:nu.over.n}
        \begin{split}
        \sum_{k=1}^m &\sum_{s,a}\frac{\nu_k(s,a)}{N_k(s,a)+1}
\leq 2\sum_{s,a} \sum_{t=1}^{T} \frac{\mathbbm{1}_{\lbrace (s_t, a_t) =(s,a)\rbrace}}{N_k(s_t,a_t)+1}
= 2 \sum_{s,a} \sum_{j=1}^{N_{T+1}(s,a)} \frac{1}{j+1} \leq 2 SA \ln(T)
\end{split}
\end{equation}


\subsubsection{Completing the proof}\label{sec:regret.summingup}
Summing up all the contributions and taking a union bound  over all possible values of $T$ and use the fact that $\sum_{T= 2}^{+\infty}\frac{\delta}{4T^{5/4}}<\delta$, we write that there exists a numerical constant $\chi$ such that at least with probability $1-\delta$ our algorithm \scalcont has a regret bounded by
\begin{align*}
        \begin{split}
                \Delta(\scalcont,T) \leq &\chi \;\left( \max{\left\lbrace \rmaxbound,c \right\rbrace} \left( S\sqrt{A T \ln\left(\frac{T}{\delta}\right)}
                        + S^2A\ln^2\left(\frac{T}{\delta} \right) 
                                          + L S^{-\alpha}T \right)
                \right)
         \end{split}
\end{align*}

We now set $S = \left(\alpha L \sqrt{\frac{T}{A}}\right)^{\sfrac{1}{(\alpha + 1)}}$ so that
\begin{align*}
    \Delta(\scalcont, T) 
    &= \wt{O} \bigg( \max\{c,\rmaxbound\} \bigg( \underbrace{\max \left\{ \alpha^{\sfrac{1}{(\alpha+1)}}, \alpha^{-\sfrac{\alpha}{(1+\alpha)}} \right \}}_{\leq 2,~\forall \alpha \geq 0} \times\\
    & \qquad \quad \times L^{\sfrac{1}{(\alpha+1)}} A^{\sfrac{\alpha}{(2\alpha+2)}} T^{\sfrac{(\alpha+2)}{(2\alpha+2)}} + \underbrace{\alpha^{\sfrac{2}{(1+\alpha)}}}_{\leq 2,~\forall \alpha >0} L^{\sfrac{2}{(1+\alpha)}} A^{\sfrac{\alpha}{(1+\alpha)}} T^{\sfrac{1}{(1+\alpha)}} \bigg ) \bigg)\\
\end{align*}
Finally, when $T \geq L^{\sfrac{2}{\alpha}}A$, the regret of \scalcont is bounded with probability at least $1-\delta$ by
\[
        \Delta(\scalcont,T) = \wt{O}\left(
            \max\{c,\rmaxbound\}L^{\sfrac{1}{(\alpha+1)}} A^{\sfrac{\alpha}{(2\alpha+2)}} T^{\sfrac{(\alpha+2)}{(2\alpha+2)}}
        \right).
\]



==> backup20180923/app_regret_continuous.tex <==
% !TEX root = main.tex
\section{Continuous state MDPs: the analysis of \scalcont} \label{app:continuous}

In all this section we say that a function $v: ~s \in \calS \mapsto \Re$ is \emph{piecewise constant on $\mathcal{I}$} when $\forall J \in \mathcal{I},~\forall s,s' \in J$ we have $v(s) = v(s') $ and we denote $v(J)$ the joint value.

\subsection{High probability bound using the exploration bonus (proof of Lem.~\ref{lem:explbonus.inequality})}\label{app:proba_bound_bonus}
To begin with, we introduce a new exploration bonus that will be useful for the regret proof:
\begin{align*}
 d_k(J,a) := c \cdot \min \left\{ \phi_{p,k}^{Ja} + \frac{1}{N_k(J,a) + 1}; 2\right\} + \min \left\{ \beta_{r,k}^{Ja}; \rmaxbound\right\} + (c + \rmaxbound)L S^{-\alpha}
\end{align*}
where
\begin{align}\label{eq:bernstein.ci.cont}
 \phi_{p,k}^{Ja} :=  \sqrt{ \frac{7 S \lnn{\frac{3 S A t_k}{\delta}}}{N_k^+(J,a)}  } + 14 S \lnn{\frac{3 S At_k}{\delta}} 
\end{align}
with $N_k^+(J,a) := \max \{1,N_k(J,a)\}$.
We define for all $(s,a)\in \calS \times \A$, $\wb{r}_k(s,a):= \wb{r}_k^{ag}(I(s), a)$.
We state a slightly more general result than Lem.~\ref{lem:explbonus.inequality}:
\begin{lemma}\label{L:bonus.inequality.continuous}
        Consider the estimated continuous MDP $\wh{M}_k$ defined in Def.~\ref{def:estimated.cont.mdp}. Let $(g^*,h^*)$ be a solution of the optimality equation $Lh^* = h^* + g^*$ such that $\SP{h^*}  \leq c$. For all $T\geq 1$, with probability at least $1-\frac{\delta}{15 t_k^6}$, for any $k \geq 1$, for any $(s,a) \in \calS \times \A$ and for any function $v$ piecewise constant on $\mathcal{I}$ \st $\SP{v} \leq c$ we have:
        \begin{align*}
                &(a)~~ \quad b_{k}(s,a) \geq \left| \wb{r}_k(s,a) - r(s,a) + \int_{\calS} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) h^*(s') \mathrm{d}s' \right|\\
                &(b)~~ \quad d_k(s,a) \geq \left| \wb{r}_k(s,a) - r(s,a) + \int_{\calS} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) v(s') \mathrm{d}s' \right|
        \end{align*}
\end{lemma}

The rest of section \ref{app:proba_bound_bonus} is devoted to proving Lem.~\ref{L:bonus.inequality.continuous}. To do this, we introduce an intermediate continuous state-space MDP $\wt{M}_k := (\calS, \A, \wt{r}_k, \wt{p}_k)$ defined for all pairs $(s,a) \in \calS \times \A$ by:
\begin{align*}
 \wt{r}_k(s,a) := \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a) r(x,a)\\
 \wt{p}_k(s'|s,a) := \frac{1}{N_k(I(s),a)}\sum_{x \in I(s)} N_k(x,a) p(s'|x,a)
\end{align*}
We decompose $\wh{p}_k -p$ as $(\wh{p}_k -\wo{p}_k) + (\wo{p}_k - \wt{p}_k) +  (\wt{p}_k -p)$ and bound separetely all the differences. Similarly, we decompose $\wh{r}_k -r$ as $(\wh{r}_k -\wt{r}_k) + (\wt{r}_k -r)$.
We also define $w^*(s) := h^*(s) - \left( \inf\{ h^*(s)\} + \sup\{ h^*(s)\} \right)/2$ implying that for all $s \in \calS$, $w^*(s) \in [-c/2, c/2]$. 

\subsubsection{Bounding the difference between $\wt{r}_k/ \wt{p}_k$ and $\wo{r}_k/ \wo{p}_k$}\label{app:bound_diff_tilde_bar}

Let's consider a fixed pair $(s,a) \in \calS \times \A$ and a fixed aggregated state $J \in \mathcal{I}$. Our first goal is to bound the differences $\int_{\calS}\big(\wt{p}_k(s'|s,a) - \wo{p}_k(s'|s,a)\big) w^*(s') \mathrm{d}s'$,~ $\int_{I}\wt{p}_k(s'|s,a) - \wo{p}_k(s'|s,a) \mathrm{d}s'$ and $\wt{r}_k(s,a) - \wo{r}_k(s,a)$ using Thm.\ref{T:inequality_stop_mds}. To do that, we need to define an adapted sequence, a sequence of stopping times and a predictable process.

\textbf{1) Adapted sequences:}\\
We will consider the following adapted sequences: $(w^*(s_t), \F_t)_{t \geq 0}$, ~$(\one{s_t \in J}, \F_t)_{t \geq 0}$ and $(r_{t-1}(s_{t-1},a_{t-1}), \F_t)_{t \geq 0}$ (with the conventions $ r_{-1}(s_{-1},a_{-1}) = r_0(s_0,a_0) = 0$, ~$w^*(s_0) = 0$ and $\one{s_0 \in J} =0$). Moreover, we also have $|w^*(s_t)| \leq 2 \times \| w^* \|_{\infty} \leq c$, ~$|\one{s_t \in J}| \leq 1$ and $|r_{t-1}(s_{t-1},a_{t-1})| \leq \rmaxbound$ for all $t \geq 0$.

\textbf{2) Stopping times:}\\
 We define $\tau := \left(\tau_l\right)_{l \geq 0}$ \st $\tau_0 := 0$ and $\inf \{ t_k > t > \tau_l : s_t \in I(s), a_t = a \}$.
%  \begin{align*}
%   \tau_{l+1} := \begin{cases}
%                  \inf \{ t_k > t > \tau_l : s_t \in I(s), a_t = a \} ~~ \text{if} ~~\{ t_k > t > \tau_l : s_t \in I(s), a_t = a \} \neq \emptyset\\
%                  \tau_l +1 ~ \text{otherwise}
%                 \end{cases}
%  \end{align*}
For all $l\geq 0$ and for all $t\geq 0$, $\tau_l :=\{ \tau_l = t \} \in \mathcal{F}_t$ and so $\tau_l$ is a stopping time \wrt $\mathbb{F}$ (see Def.~\ref{D:stop_time}). By definition for any $l \geq 0$, $\tau_l < \tau_{l+1}$ \as (\ie $\tau$ is strictly increasing). We denote $\G_l := \F_{\tau_{l\smallplus 1}}$ the \sigalg~at stopping time $\tau_{l+1}$ (see Def.~\ref{D:stop_time_algebras}).

 \textbf{3) Predictable process:}\\
 We consider the process $\big(\one{t-1 < t_k}\big)_{t \geq 0}$. It is predictable because $\{t-1 < t_k\} \in \F_{t-1}$ for all $t\geq 1$. Moreover, it is bounded by 1.
 
 All the assumptions of Thm.~\ref{T:inequality_stop_mds} are satisfied and so by taking a union bound and using the fact that $N_k(I(s),a) \leq t_k$ \as, we obtain that with probability at least $1-3\delta$ (simultaneously):
 \begin{align}
 \nonumber
  &\left| \sum_{l = 1}^{N_k(I(s),a)} \one{\tau_l < t_k}  \Big( r_{\tau_l}(s_{\tau_l},a_{\tau_l}) -\E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big]  \Big) \right| \leq \rmaxbound\sqrt{N_k(I(s),a) \lnn{\frac{2 t_k}{\delta}}}\\  
  \label{eq:bernstein_transition_proba}
  &\left| \sum_{l = 1}^{N_k(I(s),a)} \one{\tau_l < t_k}  \Big( \one{s_{\tau_l+1} \in J} - \E\big[ \one{s_{\tau_l+1} \in J} \big|\mathcal{G}_{l-1} \big] \Big) \right| \leq  2 \sqrt{V_{k}(J) \lnn{\frac{4 t_k}{\delta}}} + 4 \lnn{\frac{4t_k}{\delta}} \\ 
  \nonumber
  &\text{and}~~\left| \sum_{l = 1}^{N_k(I(s),a)} \one{\tau_l < t_k}  \Big( w^*(s_{\tau_l+1}) - \E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big] \Big) \right| \leq c \sqrt{N_k(I(s),a) \lnn{\frac{2 t_k}{\delta}}} 
 \end{align}
 where $V_k(J) := \sum_{l=1}^{N_k(I(s),a)} \one{\tau_l < t_k} \Varcond{\one{s_{\tau_l+1} \in J}}{\G_{l-1}}$.
 Note that given the definition of $\tau$, $N_k(I(s),a)= \sup \{l \geq 0: ~ \tau_l < t_k \}$ which implies that $\one{\tau_l < t_k}= 1$ for all $l \leq N_k(I(s),a)$. Therefore, we can remove the indicator function $\one{\tau_l < t_k}$ in the above sums.
 We now need to relate the above sums to $\int_{\calS}\big(\wt{p}_k(s'|s,a) - \wo{p}_k(s'|s,a) \big)w^*(s') \mathrm{d}s'$, $\int_{J}\wt{p}_k(s'|s,a) - \wo{p}_k(s'|s,a) \mathrm{d}s'$  and $\wt{r}_k(s,a) - \wo{r}_k(s,a)$. We also need to give an explicit formula for $V_k(J)$.
By defintion of $\tau$, we can rewrite $\wb{r}_k$ and $\wb{p}_k$ as follows:
\begin{align*}
   \wb{r}_k(s,a) &= \frac{1}{N_k(I(s),a)}\sum_{l=1}^{N_k(I(s),a)} r_{\tau_l}(s_{\tau_l},a_{\tau_l})\\
   \int_{J} \wb{p}_k(s'|s,a) \mathrm{d}s' &= \frac{1}{N_k(I(s),a)}\sum_{l=1}^{N_k(I(s),a)} \one{s_{\tau_l + 1} \in J}\\
   \int_{\calS} \wb{p}_k(s'|s,a) w^*(s') \mathrm{d}s' &= \frac{1}{N_k(I(s),a)}\sum_{l=1}^{N_k(I(s),a)} w^*(s_{\tau_l + 1})
\end{align*}
In order to express $\wt{p}_k$ and $\wt{r}_k$ in terms of $\E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big]$, $\E\big[ \one{s_{\tau_l+1}\in J} \big|\mathcal{G}_{l-1} \big]$ and $\E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big]$, we first prove the following useful lemma:
\begin{lemma}\label{L:conditioning_stop_time}
 For all $l \geq 1$, we have:
 \begin{enumerate}[topsep=0pt, partopsep=0pt]
 \itemsep0em 
  \item $\E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big] = \int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s' $,
  \item $\E\big[ \one{s_{\tau_l+1}\in J} \big|\mathcal{G}_{l-1} \big] = \int_{J} p(s'|s_{\tau_l},a_{\tau_l}) \mathrm{d}s' $,
  \item and  $\E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big] = r(s_{\tau_l},a_{\tau_l})$.
 \end{enumerate}
\end{lemma}
\begin{proof} To prove this result, we rely on the definition of conditional expectation (see Def.~\ref{D:cond_exp}). \\
1) By Prop.~\ref{L:process_stopped}, $(s_{\tau_l},a_{\tau_l})$ is $\G_{l-1}$-measurable ($\G_{l-1} = \F_{\tau_l}$) and so $\int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s'$ is $\G_{l-1}$-measurable too. Moreover, $\left|\int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s' \right| \leq c/2$ \as so $\int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s'$ is also integrable (and therefore $\G_{l-1}$-integrable).\\
2) We recall that for any stochastic process $(X_t)_{t\geq 0}$, we use the convention that $X_{\infty} =0$ \as implying that $X_{\tau_l} = \sum_{t=0}^{+\infty} X_t \one{\tau_l = t }$ (see Def.~\ref{D:process_stopped}). Usinng the law of total expectations (see Prop.~\ref{L:total_exp}) we have that $\forall A \in \mathcal{G}_{l-1}$,
\begin{align*}
 \E \big[ \mathbbm{1}(A) \times w^*(s_{\tau_l+1}) \big] 
 &= \sum_{t=0}^{+\infty} \E \big[  \mathbbm{1}(A \cap \{\tau_l = t \}) \times w^*(s_{\tau_l+1}) \big] \\
 &= \sum_{t=0}^{+\infty} \E \bigg[  \E \Big[ \mathbbm{1}(\underbrace{A \cap \{\tau_l = t \}}_{\in \mathcal{F}_t}) \times w^*(\underbrace{s_{\tau_l+1}}_{=s_{t+1}}) \Big| \mathcal{F}_t \Big] \bigg]
\end{align*}
In the first equality, the fact that we can move the sum outside the expectation is a direct consequence of the dominated convergence theorem (for series) since 
\begin{align*}
 \sum_{t=0}^{+\infty} \E \big[  \mathbbm{1}(A \cap \{\tau_l = t \}) \times \big|w^*(s_{\tau_l+1}) \big| \big] &\leq c/2 \sum_{t=0}^{+\infty} \E \big[  \mathbbm{1}(A \cap \{\tau_l = t \}) \big] \\&= c/2\sum_{t=0}^{+\infty} \Prob \left( A \cap \{\tau_l = t \} \right) = c/2 \cdot  \Prob (A) < +\infty
\end{align*}
Under event $\{\tau_l = t \}$ we have that $s_{\tau_l+1} = s_{t+1}$ \as Moreover, $A \cap \{\tau_l = t \} \in \F_t$ since $\tau_l$ is a stopping time (see Def.~\ref{D:stop_time_algebras}) so by Prop.~\ref{L:factor_cond_exp} we can move it outside the conditional expectation and we get:
\begin{align*}
 \E \big[ \mathbbm{1}(A) \times w^*(s_{\tau_l+1}) \big] 
 &= \sum_{t=0}^{+\infty} \E \bigg[ \mathbbm{1}(A \cap \{\tau_l = t \}) \times \underbrace{\E \Big[   w^*(s_{t+1}) \Big| \mathcal{F}_t \Big]}_{= \int_{\calS} p(s'|s_t,a_t)w^*(s')  \mathrm{d}s'} \bigg]\\
  &= \E \bigg[\mathbbm{1}(A) \times \underbrace{\sum_{t=0}^{+\infty}\mathbbm{1}(\tau_l = t ) \int_{\calS} p(s'|s_t,a_t)w^*(s')  \mathrm{d}s'   }_{=\int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s' \text{  (see Def.~\ref{D:process_stopped})}}\bigg]\\
 &= \E \left[\mathbbm{1}(A) \times \int_{\calS} p(s'|s_{\tau_l},a_{\tau_l})w^*(s')  \mathrm{d}s' \right]
\end{align*}
This proves the first inequality (see Def.~\ref{D:cond_exp}). The second and third equality can be proved using the same technique.
\end{proof}
Using Lem.~\ref{L:conditioning_stop_time} we can rewrite $\wt{r}_k$ and $\wt{p}_k$ as follows:
\begin{align*}
   \wt{r}_k(s,a) = \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} & N_k(x,a) r(x,a) = \frac{1}{N_k(I(s),a)}\sum_{l=1}^{N_k(I(s),a)} \E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big] \\ 
%    &= \frac{1}{N_k(I(s),a)}\sum_{l=1}^{T-1}  \one{\tau_l < t_k} \cdot \E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big]\\
   \text{and}~~\int_{\calS} \wt{p}_k(s'|s,a) w^*(s') \mathrm{d}s' &= \frac{1}{N_k(I(s),a)}\sum_{x \in I(s)} N_k(x,a) \int_{\calS} p(s'|x,a)w^*(s')  \mathrm{d}s'\\
   &= \frac{1}{N_k(I(s),a)} \sum_{l=1}^{N_k(I(s),a)} \E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big] \\
   \text{and similarly}~~\int_{J} \wt{p}_k(s'|s,a)  \mathrm{d}s' &= \frac{1}{N_k(I(s),a)} \sum_{l=1}^{N_k(I(s),a)} \E\big[ \one{s_{\tau_l+1} \in J} \big|\mathcal{G}_{l-1} \big]
%    &= \frac{1}{N_k(I(s),a)}\sum_{l=1}^{T - 1} \one{\tau_l < t_k} \E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big]
\end{align*}
We can also give a more explicit expression for $V_k$:
\begin{align*}
 \Varcond{\one{s_{\tau_l +1} \in J}}{\G_{l-1}} &:= \E\big[ \underbrace{\one{s_{\tau_l+1}\in J}^2}_{=\one{s_{\tau_l+1}\in J}} \big|\mathcal{G}_{l-1} \big] - \E\big[ \one{s_{\tau_l+1}\in J} \big|\mathcal{G}_{l-1} \big]^2\\
 &= \int_{J} p(s'|s_{\tau_l},a_{\tau_l}) \mathrm{d}s' - \left(\int_{J} p(s'|s_{\tau_l},a_{\tau_l}) \mathrm{d}s'\right)^2
\end{align*}
implying:
\begin{align*}
 V_k(J) = \sum_{l=1}^{N_k(I(s),a)}  \underbrace{\left( 1 - \int_{J} p(s'|s_{\tau_l},a_{\tau_l}) \mathrm{d}s' \right)}_{\leq 1} \underbrace{\int_{J} p(s'|s_{\tau_l},a_{\tau_l}) \mathrm{d}s'}_{\geq 0} \leq \sum_{x \in I(s)} N_k(x,a) \int_{J} p(s'|x,a) \mathrm{d}s'
\end{align*}
Using Cauchy-Scwartz inequality:
\begin{align*}
 \sum_{J \in \mathcal{I}} \sqrt{V_k(J)} \leq \sqrt{S \sum_{J \in \mathcal{I}} V_k(J)} \leq \sqrt{S \sum_{x \in I(s)} N_k(x,a)  \sum_{J\in \mathcal{I}}\int_{J} p(s'|x,a) \mathrm{d}s'} = \sqrt{S N_k(I(s),a) }
\end{align*}
To conclude, we take a union bound over all possible $(I(s),a) \in \mathcal{I} \times \A$ and $J \in \mathcal{I}$. Note that we only need to take a union bound over $I(s) \in \mathcal{I}$ (and not $\calS$) because $s \mapsto \wt{p}_k(\cdot|s,a)$ and $s \mapsto \wt{r}_k(s,a)$ are piecewise constant on $\mathcal{I}$ (and similarly for $\wo{p}_k$ and $\wo{r}_k$). With probability at least $1-\frac{\delta}{15 t_k^6}$, for all $(s,a) \in \calS \times \A$ and for all $J \in \mathcal{I}$:
\begin{align}
\left| \wb{r}_k(s,a) - \wt{r}_k(s,a)  \right| \leq  \rmaxbound \sqrt{\frac{\lnn{\frac{90 S^2 A t_k^7}{\delta}}}{N_k(I(s),a)} } &\leq  \rmaxbound \sqrt{\frac{7\lnn{\frac{2 S A t_k}{\delta}}}{N_k(I(s),a)} } \label{eq:hp_bound_reward}\\
 \sum_{J\in \mathcal{I}} \left|\int_{J}  \wb{p}_k(s'|s,a) - \wt{p}_k(s'|s,a)\mathrm{d}s' \right| &\leq  2 \sqrt{ \frac{7 S \lnn{\frac{3 S A t_k}{\delta}}}{N_k(I(s),a)}  } + 28 S \lnn{\frac{3 S At_k}{\delta}} \label{eq:hp_bound_proba}\\
 \left|\int_{\calS} \Big( \wb{p}_k(s'|s,a) - \wt{p}_k(s'|s,a) \Big)w^*(s') \mathrm{d}s' \right| &\leq  c \sqrt{\frac{7\lnn{\frac{2 S A t_k}{\delta}}}{N_k(I(s),a)}} \label{eq:hp_bound_proba_vector}
\end{align}
Since by definition $N_k^+(I(s),a):= \max \{ 1 , N_k(I(s),a)\}$, the above inequalities also hold with $N_k(I(s),a)$ replaced by $N_k^+(I(s),a)$.

\subsubsection{Bounding the difference between $\wt{r}_k/ \wt{p}_k$ and $r/p$}

We now bound the differences~$\wt{r}_k(s'|s,a) - r(s,a)$ and $\int (\wt{p}_k(s'|s,a) - p(s'|s,a)) w^*(s') \mathrm{d}s'$.
We use the smoothness assumption on the reward and transition model (see Asm.~\ref{asm:continuous.mdp}). For all $(s,a) \in \calS \times \A$ (using the triangle inequality):
\begin{align}\label{eq:pboundcontinuity}
\big|\wt{r}_k(s,a) - r(s,a)\big| \leq \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a) \underbrace{\big| r(x,a) -r(s,a) \big|}_{\leq \rmaxbound L S^{-\alpha} \text{ since } x,s \in I(s)} \leq \rmaxbound L S^{-\alpha}
\end{align}
For the transition probability we have that for all $J\in \mathcal{I}$ (using the triangle inequality):
\begin{align}\label{eq:pboundcontinuity3}
\begin{split}
\sum_{J \in \mathcal{I}}\left| \int_{J} (\wt{p}_k(s'|s,a) - p(s'|s,a)) \mathrm{d}s' \right| &\leq  \sum_{J \in \mathcal{I}}\int_J |\wt{p}_k(s'|s,a) - p(s'|s,a) | \mathrm{d}s'\\
         &= \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a)\int_\calS  \underbrace{|p(s'|x,a) - p(s'|s,a)|}_{\leq L S^{-\alpha} \text{ since } x,s \in I(s)} \mathrm{d}s'\\
  &\leq LS^{-\alpha}
\end{split}
\end{align}
and similarly:
\begin{align}\label{eq:pboundcontinuity2}
\begin{split}
\left|\int_\calS (\wt{p}_k(s'|s,a) - p(s'|s,a)) w^*(s') \mathrm{d}s' \right| &\leq c \int_\calS |\wt{p}_k(s'|s,a) - p(s'|s,a) | \mathrm{d}s'\\
         &= \frac{c}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a)\int_\calS  \underbrace{|p(s'|x,a) - p(s'|s,a)|}_{\leq L S^{-\alpha} \text{ since } x,s \in I(s)} \mathrm{d}s'\\
  &\leq cLS^{-\alpha}
\end{split}
\end{align}

\subsubsection{Bounding the difference between $\wh{p}_k$ and $\wo{p}_k$}\label{app:bound_diff_hat_bar}
Using the triangle inequality we have that for any $(s,a) \in \calS \times \A$:
\begin{align}\label{eq:p.bound.perturbation.cont}
\begin{aligned}
\left|\int_{\calS} (\wh{p}_k(s'|s,a) - \wb{p}_k(s'|s,a)) w^*(s') \mathrm{d}s' \right| &\leq  \int_{\calS} \left|\wh{p}_k(s'|s,a) - \wb{p}_k(s'|s,a) \right| \cdot\left| w^*(s') \right|\mathrm{d}s'  \\
&= \left| \frac{N_k(I(s),a) }{N_k(I(s),a)+1} - 1 \right| \int_\calS \wb{p}_k(s'|s,a) \underbrace{|w^*(s')|}_{\leq c/2} \mathrm{d}s'\\ &~~~+ S\int_\calS \frac{|w^*(s')|\mathbbm{1}(s' \in I(\wb{s}))}{N_k(I(s),a) + 1} \mathrm{d}s'\\ 
&\leq \frac{c}{N_k(I(s),a) + 1}
\end{aligned}
\end{align}
and similarly:
\begin{align}\label{eq:p.bound.perturbation.cont2}
\begin{aligned}
\sum_{J\in \mathcal{I}}\left|\int_{J} (\wh{p}_k(s'|s,a) - \wb{p}_k(s'|s,a))  \mathrm{d}s' \right| \leq \int_{\calS} \left|\wh{p}_k(s'|s,a) - \wb{p}_k(s'|s,a)  \right|\mathrm{d}s' \leq \frac{1}{N_k(I(s),a) + 1}
\end{aligned}
\end{align}

\subsubsection{Gathering all the terms}

We first notice that $\int_{\calS} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) h^*(s')\mathrm{d}s' = \int_{\calS} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) w^*(s')\mathrm{d}s'$ since $w^*$ and $h^*$ are equal up to a constant shift and $\int_{\calS}\wh{p}_k(s'|s,a) \mathrm{d}s'= \int_{\calS}{p}(s'|s,a)\mathrm{d}s' = 1$. Gathering equations \eqref{eq:hp_bound_proba_vector}, \eqref{eq:pboundcontinuity2} and \eqref{eq:p.bound.perturbation.cont} we have:
\begin{align*}
 \left| \int_{\calS} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) h^*(s')\mathrm{d}s' \right| \leq c \sqrt{\frac{7\lnn{\frac{2 S A t_k}{\delta}}}{N_k^+(I(s),a)}} + cL S^{-\alpha} + \frac{c}{N_k(I(s),a) + 1}
\end{align*}
Gathering equations \eqref{eq:hp_bound_reward} and \eqref{eq:pboundcontinuity} we have:
\begin{align*}
 \left| \wb{r}_k(s,a) - r(s,a) \right| \leq \rmaxbound \sqrt{\frac{7\lnn{\frac{2 S A t_k}{\delta}}}{N_k^+(I(s),a)} } + \rmaxbound LS^{-\alpha} 
\end{align*}

Let $v$ be a piecewise constant function on $\mathcal{I}$ \st $\SP{v} \leq c$ and define $w(s) := v(s) - \left( \inf\{ v(s)\} + \sup\{ v(s)\} \right)/2$. $w$ is also piecewise constant on $\mathcal{I}$ and for all $J \in \mathcal{I}$, $w(J) \in [-c/2, c/2]$.  Gathering equations \eqref{eq:hp_bound_proba}, \eqref{eq:pboundcontinuity3} and \eqref{eq:p.bound.perturbation.cont2} we have that :
\begin{align*}
 \sum_{J \in \mathcal{I}}\left| \int_{J} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) v(s') \mathrm{d}s' \right| &= \sum_{J \in \mathcal{I}}\left| w(J) \int_{J} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) \mathrm{d}s' \right| \\
 & \leq \frac{c}{2} \sum_{J \in \mathcal{I}}\left| \int_{J} \left( \wh{p}_k(s'|s,a) - p(s'|s,a) \right) \mathrm{d}s' \right|\\
 & \leq c \sqrt{ \frac{7S \lnn{\frac{3 S A t_k}{\delta}}}{N_k^+(I(s),a)}  } + 14 c S \lnn{\frac{3 S At_k}{\delta}} + cL S^{-\alpha} \\&~~~~+ \frac{c}{N_k(I(s),a) + 1}
\end{align*}
Properties \emph{(a)} and \emph{(b)} of Lem.~\ref{L:bonus.inequality} follow by definition of the exploration bonuses and application of the triangle inequality.

\subsection{Optimism (Proof of Lem.~\ref{L:optimism})}

Let $\wh{g}^{ag+}_k$ denote the solution of optimisation problem \eqref{eq:opt.superior.spanc} on $\wh{M}^{ag+}_k$. In this section we prove that:
\begin{lemma}\label{L:optimism.cont}
        Consider the MDP $\wh{M}^{ag+}_k$ defined in Sec.~\ref{S:exploration.bonus.continuous}. Then for any $k>0$, with probability at least $1-\frac{\delta}{15 t_k^6}$, $\wh{g}^{ag+}_k \geq g^*$.
\end{lemma}
$\wh{M}^{ag+}_k$ only has a finite number of states while the true MDP $M^*$ has an uncountable state-space. Thus, it is difficult to compare directly $\wh{g}^{ag+}_k$ with $g^*$. To overcome this difficulty, we first compare $g^*$ with the gain of $\wh{M}_k$ and then compare the latter to $\wh{g}^{ag+}_k$.
% The proof is divided into three parts. 
% The first part shows that a continuous MDP $\wh{M}_k = (\calS,\A, \wh{p}_k, \wh{r}_k)$ constructed using the observed samples and the exploration bonus $b_k$ is optimistic \wrt the true MDP $M^*$.
% In the second part we show that the discrete MDP $\wh{M}^{ag}_k = (\mathcal{I}, \A, \wh{p}_k^{ag}, \wh{r}^{ag}_k)$ has the same gain of the continuous MDP $\wh{M}_k$ and thus it is optimistic.
% Finally, we show that the augmented MDP $\wh{M}^{ag+}_k$ is optimistic.

\paragraph{1. Optimism of $\wh{M}_k$.}
Let $\wh{g}_k$ denote the solution of optimisation problem \eqref{eq:opt.superior.spanc} on $\wh{M}_k$. % instead of $\wh{M}^{+}_k$.
To prove that $\wh{g}_k \geq g^*$ we can use Prop.~\ref{prop:bound.gain} which --as explained in the main body of the paper-- only requires to show that $\wh{L}_kh^* \geq Lh^*$ where $\wh{L}_k$ is the optimal Bellman operator of $\wh{M}_k$. By applying property \emph{(a)} of Lem.~\ref{L:bonus.inequality.continuous}, we have that with probability at least $1-\frac{\delta}{15 t_k^6}$:
\begin{align*}
    \forall s\in \calS,~\wh{L}_k h^*(s) &:= \max_{a \in \A} \left\{ \wb{r}_k(s,a) + b_k(s,a) + \int_{\calS} \wh{p}_k(s'|s,a) h^*(s') \mathrm{d}s' \right\}\\
                 &\geq \max_{a\in\A} \left\{ r(s,a) + \int_{\calS} p(s'|s,a) h^*(s') \mathrm{d}s'\right\} = Lh^*(s) 
\end{align*}
Therefore, $\wh{g}_k \geq g^*$ with probability at least $1-\frac{\delta}{15 t_k^6}$.


\paragraph{2. Relationship between $\wh{M}_k$ and $\wh{M}^{ag+}_k$.} 
% The optimism we have proved is between the true MDP and a continuous MDP using the exploration bonus.
% In practice, we are not planning using $\wh{M}_k$ but using the discrete MDP $\wh{M}^{ag}_k$.
% Recall that $\wh{M}^{ag}_k = (\mathcal{I}, \A, \wh{p}_k^{ag}, \wh{r}^{ag}_k)$ where $\wh{p}_k^{ag}$ and $\wh{r}_k^{ag}$ are defined in Sec.~\ref{S:exploration.bonus.continuous}.
We now show that $\wh{g}^{ag+}_k = \wh{g}_k$.
Consider a piecewise-constant function $v_0$ on $\mathcal{I}$ (\eg $v_0 = 0$) and a vector $u_0 \in \Re^S$ satisfying $u_0(J) = v_0(J)$ for all $J \in \mathcal{I}$. We define the sequences $v_{n+1} := \wh{T}_c v_n$ and $u_{n+1} := \wh{T}_c^{ag+} u_n$. We show by induction that $u_n(J) = v_n(J)$ for all $n \geq 0$ and for all $J \in \mathcal{I}$. By definition it is true for $n=0$ and for all $n \geq 0$:
\begin{align}\label{eq:piecewise_vector_proba}
\begin{split}
   \int_{s \in \calS} \wh{p}_k(s'|s,a) v_n(s') \mathrm{d}s' 
       &= \sum_{J \in \mathcal{I}} \int_{J} \wh{p}_k(s'|s,a) v_n(s') \mathrm{d}s'\\
       &= \sum_{J \in \mathcal{I}} v_n(J) \int_{J} \wh{p}_k(s'|s,a)\mathrm{d}s' = \sum_{J \in \mathcal{I}} u_{n}(J)\; \wh{p}^{ag}_k(J| I(s),a)
\end{split}
\end{align}
where the last equality follows from \eqref{eq:integral.p.perturbed} and the induction hypothesis.
In addition $\wh{r}_k(s,a)$ is also piecewise-constant on $\mathcal{I}$ and $\wh{r}_k(s,a) = \wh{r}^{ag}_k(I(s),a)$ for all $s \in \calS$. Therefore, we have that $\wh{L}^{ag}_k u_n(I(s)) = \wh{L}_k v_n(s)$ for any $s \in \calS$. Finally, the augmentation is not impacting the optimal Bellman operator (\ie for any $v$, $\wh{L}^{ag+}_k v = \wh{L}^{ag}_kv$) so $\wh{L}^{ag+}_k u_n(I(s)) = \wh{L}_k v_n(s)$ and consequently $\wh{T}^{ag+}_c u_n(I(s)) = \wh{T}_c v_n(s)$ for any $s \in \calS$. This shows that $v_{n+1}(J) =u_{n+1}(J)$ for all $J \in \mathcal{I}$ which concludes the proof by induction.

As shown by \citet[Theorem 10]{fruit2018constrained}, $ \lim_{n \to +\infty}v_{n+1}(J) - v_n(J) = \wh{g}^{ag+}_k$ and $ \lim_{n \to +\infty}u_{n+1}(J) - u_n(J) = \wh{g}_k$ so that $\wh{g}^{ag+}_k = \wh{g}_k \geq g^*$ with probability at least $1-\frac{\delta}{15 t_k^6}$.
% Thus,  $\forall s \in \calS$, $\wh{T}_c^{ag} v_n(I(s)) = \wh{T}_c v_n(s)$ and $g^*_c(\wh{M}_k^{ag}) = g^*_c(\wh{M}_k) \geq g^*$ w.h.p.
% Since the augmentation is not changing the application of the Bellman operator (\ie for any $v$, $\wh{L}^{ag+}_k v = \wh{L}^{ag}_kv$)  we have that $g^*_c(\wh{M}^{ag+}_k) = g^*_c(\wh{M}^{ag}_k)$
% and the fact that $\wh{p}^{ag}_k = \wh{p}^{ag+}_k$ (by definition)
% 
% \paragraph{3. The reward augmentation.} 
% We now need to relate the optimal gains of $\wh{M}^{ag+}_k$ and $\wh{M}^{ag}_k$. 
% Since the augmentation is not changing the application of the Bellman operator (\ie for any $v$, $\wh{L}^{ag+}_k v = \wh{L}^{ag}_kv$)  we have that $g^*_c(\wh{M}^{ag+}_k) = g^*_c(\wh{M}^{ag}_k) = g^*_c(\wh{M}_k) \geq g^*$ w.h.p.


==> backup20180923/app_regret_finite.tex <==
% !TEX root = main.tex
\section{Discrete MDPs: the analysis of \bonusscal}\label{app:finite}
In this section we analyse \bonusscal by leverages the results provided for the continuous state case.
We start presenting the derivation of the bonus $b_k$ and an analogous of Lem.~\ref{L:bonus.inequality.continuous} which implies \bonusscal is optimistic at each episode $k$.
Finally, we provide a proof of the regret bound stated  in Thm.~\ref{thm:regret.scalcont}.

\subsection{High probability bound using the exploration bonus (proof of Lem.~\ref{lem:explbonus.inequality})}\label{app:proba_bound_bonus.discrete}

To begin with, we introduce a new exploration bonus that will be useful for the regret proof:
\begin{align*}
 d_k(s,a) := c \cdot \min \left\{ \phi_{p,k}^{sa} + \frac{1}{N_k(s,a) + 1}; 2\right\} + \min \left\{ \beta_{r,k}^{sa}; \rmaxbound\right\}
\end{align*}
where
\begin{align*}
 \phi_{p,k}^{sa} := \sqrt{\frac{7 (\Gamma -1)\lnn{\frac{3 SA t_k}{\delta}}}{N_k^+(s,a)}} + \frac{14S}{N_k^+(s,a)} \lnn{\frac{3SAt_k}{\delta}}
\end{align*}
Notice that compared to the bonus $b_k$, $d_k$ explicitly depends on the number of states (linearly in $S$) and next states (sublinearly in $\Gamma$).
As a consequence, $d_k(s,a) \geq b_k(s,a)$ for any $(s,a) \in \calS \times \A$.
{\color{red} In the continuous case we might consider the number of next states in the (true) aggregated MDP. However, this quantity is not very informative so we have decided (for sake of clarity) to upper-bound it by the number of intervals.}


\begin{lemma}\label{L:bonus.inequality}
        Let $(g^*,h^*)$ be a solution of the optimality equation $Lh^* = h^* + g^*$ such that $\SP{h^*}  \leq c$. For all $T \geq 1$, with probability at least $1-\frac{\delta}{15 t_k^6}$, for any $k \geq 1$, for any $(s,a) \in \calS \times \A$ and for any $v \in \mathbb{R}^S$ \st $\SP{v} \leq c$ we have:
        \begin{align*}
                &(a) ~~ b_{k}(s,a) \geq \left| \wb{r}_k(s,a) - r(s,a) + \left( \wh{p}_k(\cdot|s,a) - p(\cdot|s,a) \right)^\transp h^* \right|\\
                &(b) ~~ d_k(s,a) \geq \left| \wb{r}_k(s,a) - r(s,a) + \left( \wh{p}_k(\cdot|s,a) - p(\cdot|s,a) \right)^\transp v \right|
        \end{align*}
\end{lemma}
\begin{proof}
        We consider the discrete case as a special sub-case of the continuous one considered in Lem.~\ref{L:bonus.inequality.continuous}.
        \todom{Note that for the discrete case we can even use an independence argument based on ``stack of samples'' idea as done for bandits~\citep[][Sec. 4.4]{bandittorcsaba}. However, for sake of clarity we use the same MDS argument exploited in the continuous case.}
        The main difference is that in the discrete case we do not need state aggregation and thus we replace every interval with a singleton function, \ie $I(s) = s,~\forall s \in \calS$.
        Define $w := h - (\min\{h\} + \max\{h\})/2$ such that $w \in [-c/2, c/2]$.
        We decompose $\wh{p}_k -p$ into $(\wh{p}_k - \wb{p}_k) + (\wb{p}_k - p)$. As done in Eq.~\ref{eq:p.bound.perturbation.cont} (Sec.~\ref{app:bound_diff_hat_bar}), we can write that
        \begin{equation}\label{eq:bound.perturbation.p}
        \begin{aligned}
                \big|  (\wh{p}_k(\cdot|s,a) - \wb{p}_k(\cdot|s,a) )^\transp w \big| 
                % &= \left| \left(\frac{N_k(s,a)}{N_k(s,a)+1} -1 \right)\wb{p}_k(\cdot|s,a)^\transp w +  \frac{w(\wb{s})}{N_k(s,a)+1}  \right|\\
                &\leq \left|\frac{N_k(s,a)}{N_k(s,a)+1} -1 \right| \underbrace{\|\wb{p}_k(\cdot|s,a)\|_1}_{=1} \underbrace{\|w\|_{\infty}}_{\leq c/2} +\frac{|w(\wb{s})|}{N_k(s,a)+1} \\
                &\leq \frac{c}{2} \left( 1 - \frac{N_k(s,a)}{N_k(s,a)+1} + \frac{1}{N_k(s,a)+1} \right)
                = \frac{c}{N_k(s,a) + 1} 
        \end{aligned}
        \end{equation}
        %
        In order to bound the term depending on $(\wb{p}_k - p)$ we use the same MDS argument as in Sec.~\ref{app:bound_diff_tilde_bar}.
        You can consider $p$ equivalent to $\wt{p}$ defined in the continuous case since:
        \[
                \wt{r}_k(s,a) = \frac{1}{N_k(\underbrace{I(s)}_{:=s},a)} \sum_{x \in \underbrace{I(s)}_{:=s}} N_k(x,a) r(x,a) = r(s,a).
        \]
        Similarly, we can prove that $\wt{p}_k(s'|s,a) = p(s'|s,a)$. Then, we consider the same adapted sequences, stopping times and predictable processes except from the fact that intervals are replaced by singletons (\ie discrete states).
        As a consequence, (an analogous of) Lem.~\ref{L:conditioning_stop_time} holds.
        %$\forall l \geq 1$, $\E\big[ w^*(s_{\tau_l+1}) \big|\mathcal{G}_{l-1} \big] = p(\cdot|s_{\tau_l},a_{\tau_l})^\transp w^*$,
        %$\E\big[ \one{s_{\tau_l+1} = s'} \big|\mathcal{G}_{l-1} \big] = p(s'|s_{\tau_l},a_{\tau_l})$, and $\E\big[ r_{\tau_l}(s_{\tau_l},a_{\tau_l}) \big|\mathcal{G}_{l-1} \big] = r(s_{\tau_l},a_{\tau_l})$ 
        By following the same steps in Sec.~\ref{app:bound_diff_tilde_bar}, we can prove that with probability at least $1-\delta$, for all $(s,a) \in \calS \times \A$
        \begin{align*}
                \left| \wb{r}_k(s,a) - r_k(s,a)  \right| &\leq  \rmaxbound \sqrt{\frac{7\lnn{\frac{2 S A T}{\delta}}}{N_k^+(s,a)} } := \beta_{r,k}^{sa} \\
                \left|\big( \wb{p}_k(\cdot|s,a) - p(\cdot|s,a) \big)^\transp w^* \right| &\leq  c \sqrt{\frac{7\lnn{\frac{2 S A T}{\delta}}}{N_k^+(s,a)}} := \beta_{p,k}^{sa}
        \end{align*}
        where we recall the $N_k^+(s,a) := \max\{1, N_k(s,a)\}$.
        We now consider the concentration of $(\wh{p}_k -p)^\transp v$ for which we need to use Freedman's inequality (see Thm.~\ref{T:inequality_stop_mds}).
        Similarly to what done before, let $z = v - (\min\{v\} + \max\{v\})/2$ such that $(\wh{p}_k - p)^\transp v = (\wh{p}_k - p)^\transp z$. 
        We start noticing that, Eq.~\ref{eq:bernstein_transition_proba} holds for the discrete case where we replace the adapted sequence $\one{s_{\tau_l+1} \in I}$ by $\one{s_{\tau_l+1} \in I}$ 
        and the conditional variance $V_k(J)$ by $V_k(s') = \sum_{l=1}^{N_k(s,a)} \one{\tau_l < t_k} \Varcond{\one{s_{\tau_l+1} =s'}}{\G_{l-1}}$.
        Furthermore, $\Varcond{\one{s_{\tau_l+1} = s'}}{\mathcal{G}_{l-1}} = (1-p(s'|s,a)) p(s'|s,a)$ and
        \[
                V_k(s') = \sum_{l=1}^{N_k(s,a)} (1 - p(s'|s_{\tau_l}, a_{\tau_l})) p(s'|s_{\tau_l},a_{\tau_l}) \leq N_k(s,a) (1 - p(s'|s,a)) p(s'|s,a) 
        \]
        As done in~\citep[][App. F.7]{fruit2018constrained} we use Cauchy-Schwartz inequality to write that
        \begin{align*}
                \sum_{s' \in \mathcal{S}} \sqrt{p(s'|s,a)(1-p(s'|s,a))} &= \sum_{s' \in \mathcal{S}:~ p(s'|s,a)>0} \sqrt{p(s'|s,a)(1-p(s'|s,a))} \leq \sqrt{\Gamma -1}
        \end{align*}
        where we recall that $\Gamma := \max_{s,a} \| p(\cdot|s,a) \|_0$ is the maximum support of $p$.
        Then, for any $(s,a) \in \calS \times\A$ and for any vector $z \in [-c/2,c/2]$, we have that
        \begin{align*}
                \left|\big(\wb{p}_k(\cdot|s,a) - p(\cdot|s,a) \big)^\transp z\right| 
                &\leq \|z\|_{\infty}\sum_{s' \in \calS} |\wb{p}_k(s'|s,a) - p(s'|s,a)| \\
                &\leq \frac{c}{2 N_k^+(s,a)} \sum_{s' \in \calS} \left(2 \sqrt{V_{k}(s') \lnn{\frac{4 t_k}{\delta}}} + 4 \lnn{\frac{4t_k}{\delta}} \right)\\
                &\leq c  \left( \sqrt{\frac{7 (\Gamma -1)\lnn{\frac{3 SA t_k}{\delta}}}{N_k^+(s,a)}} + \frac{14S}{N_k^+(s,a)} \lnn{\frac{3SAt_k}{\delta}} \right)
                := c\; \phi_{p,k}^{sa}
        \end{align*}
        %
        We can also write with probability $1$ that:
        \begin{align*}
                \big| (\wh{p}_k(\cdot|s,a) - p(\cdot|s,a) )^\transp w \big|
                \leq \wh{p}_k(\cdot|s,a) ^\transp w +  p(\cdot|s,a)^\transp w 
                 \leq 2 c
        \end{align*}
        So we can take the minimum between the two upper-bounds. We also know that the difference in reward is bound by $\rmaxbound$.
%         The results follow by taking a union bound over all possible state-action pairs $(s,a) \in \calS \times \A_s$ and possible values of $N_k(s,a) = 0, \dots, t_k -1$:
%         \begin{align*}
%          \sum_{s,a} \sum_{N_k(s,a) = 0}^{t_k - 1} \left( \frac{\delta}{60 t_k^7 S A} + \frac{\delta}{20 t_k^7 S A} \right) \leq \frac{\delta}{15 t_k^6}.
%         \end{align*}
\end{proof}

% We can finally prove that $g^*_c(\wh{M}_k^+) = \max_{\pi \in \PiC(\wh{M}_k^+)} \{ g^\pi_{\wh{M}_k^+} \}$ is optimistic \wrt $g^* = \max_{\pi \in \SD} \{g^\pi_{M^*}\}$.
In order to prove optimism we start noticing that the bonus $b_k(s,a)$ (see Lem.~\ref{L:bonus.inequality}) implies that $\wh{L}_k h^* \geq Lh^*$. As a consequence, we can use Prop.~\ref{prop:bound.gain} to show that $g^+_k \geq g^*$.

\subsection{Regret Proof of \bonusscal}
The regret proof follows the same steps of the one for \scalcont.
The main difference resides in the fact that there is no need of state aggregation, \ie simplifying the proof.

By using the optimism of $\wh{M}^+_k$,  the stopping condition of \scopt and the relationships between $\wh{M}^+_k$ and $\wh{M}_k$ (see Eq.~\ref{eq:mdp.augmentation.props}), we can prove Eq.~\ref{eq:deltak.bound} for the discrete case.
Note that the analysis of the cumulative contribution of the term $d_k(s,a)$ and $b_k(s,a)$ will lead to the following terms $\wt{O}(c\sqrt{\Gamma SAT})$ and $\wt{O}(c \sqrt{SAT})$, respectively. Since the dominant term is the one associated to $d_k$, even in this case we upper-bound $b_k$ by $d_k$.

From this point, we follow the same steps as in Sec.~\ref{app:proof.regret.continuous}. The only difference resides in Eq.~\ref{eq:sum.deltak} where the term $(c + \rmaxbound) LS^{-\alpha} T$ disappears since it depends on aggregation and/or smoothness.
Finally, the regret bound in Thm.~\ref{thm:regret.bonusscal} follows by noticing that the order of the term $\sum_{k=1}^m \sum_{s,a} \nu_k(s,a) \phi_{p,k}^{sa}$ is $\wt{O}(c\sqrt{\Gamma S A T} + S^2 A)$.

As a consequence, there exists a numerical constant $\chi$ such that at least with probability $1-\delta$ our algorithm \bonusscal has a regret bounded by
\begin{align*}
        \begin{split}
                \Delta(\bonusscal,T) \leq &\chi \;\left( \max{\left\lbrace \rmaxbound,c \right\rbrace} \left( \sqrt{\Gamma S A T \ln\left(\frac{T}{\delta}\right)}
                        + S^2A\ln^2\left(\frac{T}{\delta} \right) 
                                          \right)
                \right)
         \end{split}
\end{align*}



==> backup20180923/sec_bonus_finite.tex <==
% !TEX root = main.tex
\section{\bonusscal: \scal with exploration bonus}
\label{S:exploration.bonus}

\todor{Intro of section}

\subsection{The algorithm}
\bonusscal proceeds through episodes $k=1,2,\ldots$ Denote by  $N_k(s,a,s')$ the number of observations of 3-tuples $(s,a,s')$ before episode $k$ ($k$ excluded) and by $N_k(s,a) := \sum_{s'}N_k(s,a,s')$ the number of visits in state-action pair $(s,a)$ before $k$. We define $\wo{r}(s,a)$ and $\wo{p}(\cdot|s,a)$ the empirical averages of $r$ and $p$ respectively:
\begin{align*}
        \wo{p}_k(s'|s,a) := \frac{N_k(s,a,s')}{N_k(s,a)}  ~~\text{ and }~~  \wo{r}_k(s,a) := \frac{1}{N_k(s,a)} \sum_{t=1}^{t_k -1} r_t(s_t,a_t) \mathbbm{1}(s_t,a_t = s,a).
\end{align*}

We define $\wh{M}_k := (\calS, \A, \wh{p}_k, \wh{r}_k)$ where $\wh{r}_k = \wo{r}_k + b_k$ (with $b_k$ a suitable exploration bonus defined later) and
% \begin{equation}\label{E:hatp}
%         \wh{p}_k(s'|s,a) = \begin{cases}
%                 \frac{N_k(s,a,s')+1}{N_k(s,a) + 1} & \textit{if  }s' = \wb{s}\\
%                 \frac{N_k(s,a,s')}{N_k(s,a) + 1}  & \textit{otherwise}
%         \end{cases}
% \end{equation}
\begin{equation}\label{E:hatp}
        \wh{p}_k(s'|s,a) = \frac{N_k(s,a) \wo{p}_k(s'|s,a)}{N_k(s,a) + 1} +   \frac{\mathbbm{1}(s'= \wb{s}) }{N_k(s,a) + 1}
\end{equation}
is a biased (but asymptotically consistent) estimator of the probability of transition $(s,a) \mapsto s'$.
At the beginning of each episode $k$, \bonusscal builds the \emph{augmented} MDP $\wh{M}_k^+ = (\calS, \A^+, \wh{p}_k^+, \wh{r}_k^+)$ where each action in $\wh{M}_k$ is duplicated with transition probability unchanged and reward set to $0$. Formally, $\A^+ = \A \times \{1, 2 \} $ and for the sake of clarity, we denote any $(a,i) \in \A \times \{1,2\}$ by $a_i$. We then define $\wh{p}_k^+(s'|s,a_i) := \wh{p}_k(s'|s,a)$ and $\wh{r}_k^+(s,a_i) := \wh{r}_k(s,a) \cdot \mathbbm{1}(i=1)$

The small bias in the empirical estimate $\wh{p}_k$ of the transition probabilities ensures that the ``\emph{attractive}'' state $\wb{s}$ is reached with non-zero probability from any state-action pair $(s,a_i)$ implying that the \emph{ergodic coefficient} of $\wh{M}_k^+$
\[
\gamma_k = 1 - \min_{
        \substack{
s,u \in \mathcal{S},\\ a, b \in \mathcal{A}
}
} 
\bigg\{ \sum_{j \in \calS}\underbrace{\min \left\{ \wh{p}_k(j|s,a),\wh{p}_k(j|u,b) \right\}}_{\geq \eta_k := \min_{s,a}\left\{ \frac{N_k(s,a,\wb{s}) + 1}{N_k(s,a) + 1}\right\} >0 ~\text{if}~ j=\wb{s}} \bigg\}
\]
is smaller than $1-\eta_k <1$ and thus the Bellman operator of $\wh{M}_k^+$, denoted $\wh{L}^+$, is $\gamma_k$-contractive~\citep[Thm. 6.6.6]{puterman1994markov}. Moreover, state $\overline{s}$ necessarily belongs to all \emph{recurrent classes} of all policies implying that $\wh{M}_k^+$ is unichain. Note that a similar trick is used in \scal~\citep{fruit2018constrained} to ensure that the ergodic coefficient is strictly smaller than 1. Instead of biasing the \emph{estimated} transition probabilities, \scal only \emph{perturbs} (\ie~biases) the \emph{optimistic} transition probabilities. 

By \emph{augmenting} the rewards, we ensure that for all $v$ such that $\SP{v} \leq c$, $\wh{T}_{c}^+$ is globally feasible at $v$ (refer to Lem. 5 of~\citet{fruit2018constrained}).
Therefore, Asm. 6 and 9 of~\citet{fruit2018constrained} are satisfied by $\wh{M}_k^+$ thus Lem. 8 and Thm. 10 hold \ie~ \scopt applied to $\wh{M}_k^+$ always stops in a finite number of iterations and returns an $\epsilon_k$-approximate solution of the optimality equation associated to $\wh{T}_{c}^+$ . 

\bonusscal is a variant of \scal that applies \scopt on the MDP $\wh{M}_k^+$ (instead of a bounded parameter MDP) at each episode $k$ in order to (approximately) solve the optimization problem~\ref{eq:opt.superior.spanc} on $\wh{M}_k^+$.
% \begin{equation}\label{eq:scalp.optimization}
%         \max_{\pi \in \PiC(\wh{M}_k^+)} g_{\wh{M}_k^+}^\pi
% \end{equation}
% whose maximum is denoted by $\wh{g}^+_k$.
\scopt is run with an initial value function $v_0 = 0$, the same reference state $\wb{s}$ that is used to construct $\wh{p}_k^+$, contraction factor $\gamma_k = 1 -\eta_k$, and accuracy $\epsilon_k = \sfrac{\rmaxbound}{\sqrt{t_k}}$.
\scopt finally returns an \emph{optimistic} (nearly) optimal policy $\wt{\pi}_k$ 
% ($g^{\wt{\pi}_k}(\wh{M}^+_k) \geq g^*_{M} - \epsilon_k$) 
satisfying the span constraint. 
Note that policy $\wt{\pi}_k$ takes action in the augment set $\A^+$, its projection to $\A$ is simply  $\wt{\pi}_k(s,a) \leftarrow \wt{\pi}_k(s,a_1) + \wt{\pi}_k(s,a_2)$, for all $s \in \calS, a \in \A_s$ (we use the same notation for the two policies).
Policy $\wt{\pi}_k$ is executed until the end of the episode.

\input{algo_bonus}

\subsection{Optimistic Exploration Bonus}\label{sec:exploration_bonus}

{\color{red} TODO: simplify the explanation of the proof of optimism (harmonize notations...). Move the definition of the bonus to section 3.1.}

All algorithms relying on the OFU principle (\eg~ \ucrl, \optpsrl, \scal, etc.) have the property that the optimal gain of the MDP used for planning is an upper bound on the optimal gain of the true MDP $g^*$. This is a key step in deriving regret guarantees.
If we want to use the same proof technique for \bonusscal, we also have to ensure that the policy $\wt{\pi}_k$ is \emph{gain-optimistic} (up to an $\varepsilon_k$- accuracy), \ie $\wh{g}^+_k \geq g^* $.

To enforce Lem.~\ref{L:optimism}, we need to tailor the exploration bonus accordingly. 
\ucrl plans in an extended MDP that ``contains'' the true MDP $M$ (with high probability) which immediately implies that (an analogue of) Lem.~\ref{L:optimism} holds (for the extended MDP instead of $\wh{M}_k^+$). A similar argument is used for \scal. Unfortunately, we never defined any ``extended MDP'' or set of ``plausible MDPs'' for \bonusscal and so we cannot apply the same reasoning.
To prove Lem.~\ref{L:optimism}, we will rather rely on Lem. 8 in~\citep{fruit2018constrained} (inspired by Thm. 8.4.1.c in~\citep{puterman1994markov}). In particular, we leverage on the dominance property: 
\begin{proposition}\label{prop:bound.gain}
Denote by $g^+$ the gain associated to operator $\opT{}$.
If there exists $(g,h)$ satisfying $\opT{h} \geq h + ge$ then $g^+ \geq g$.
\end{proposition}
\begin{proof}
By induction, using the monotonicity and linearity of $ {T}_c$ \citep[Lemma 16 (a) \& (c)]{fruit2018constrained}, we have that
$
    \forall n \in \mathbb{N},~~({T}_c)^{n+1} h \geq ({T}_c)^{n} h + ge
$.
By Lemma 8 and Theorem 10 of \citet{fruit2018constrained}, $\lim_{n \to + \infty} ({T}_c)^{n+1} h - ({T}_c)^{n} h = g^+$. Taking the limit when $n$ tends to infinity in the previous inequality yields: $g^+ \geq g$.
\end{proof}
%To prove Lem.~\ref{L:optimism}, we will rather rely on the following proposition proved by \citet{fruit2018constrained} and inspired by Theorem 8.4.1.c in~\citet{puterman1994markov}.
%\begin{proposition}\label{prop:bound gain}
% Let $M$ be an MDP satisfying Asm. 6 of \citep{fruit2018constrained} and $\opT{}$ the operator introduced in Def. 1 of \citep{fruit2018constrained}. Denote by $g^+$ the gain associated to operator $\opT{}$.
% If there exists $(g,h)$ satisfying $\opT{h} \geq h + ge$ then $g^+ \geq g$.
%\end{proposition}
Recall that the optimal gain and bias of the true MDP $(g^*,h^*)$ satisfy the optimality equation $Lh^* = h^* + g^* e$. Since in addition $\SP{h^*} \leq c$ (by assumption), we also have $\SP{L h^*} = \SP{h^* + g^* e} = \SP{h^*} \leq c$ and so $\opT{h^*} = L h^*$.
We know from Theorem 10 of \citet{fruit2018constrained} that $\wh{g}^+_k$ is the gain of operator $\wh{T}_{c}^+$ and so according to Prop.~\ref{prop:bound.gain}, it is sufficient to show that $\wh{T}_{c}^+ h^* \geq h^* + g^* e = \opT{h^*} $ to prove Lem.~\ref{L:optimism}.
\citet[Lemma 15]{fruit2018constrained} also showed that the projection $\proj{}$ (see Eq.~\ref{eq:opT}) is monotone implying that a sufficient condition for $\proj{\wh{L}^+h^*} = \wh{T}_{c}^+ h^* \geq \opT{h^*} = \proj{\wh{L}h^*}$ to hold is to have $\wh{L}^+ h^* \geq L{h^*} $. To guarantee that the inequality holds with high probability, we have to properly scale the exploration bonus.
%
Based on Hoeffding's inequality we define the quantities
\begin{align}\label{eq:confidence.intervals}
\beta_{p,k}^{sa}
&:= 
\sqrt{\frac{7 \ln \left( 2SAt_k/ \delta\right)
                }{\max\lbrace 1, N_k(s,a)\rbrace}} ~~ \text{ and } ~~
\beta_{r,k}^{sa}
:= \rmaxbound \; \beta_{p,k}^{sa}
\end{align}
% where $b_{k,\delta} = \ln \left( 2SAt_k/ \delta\right)$ is just a logarithmic term.
Then, the exploration bonus $b_k(s,a)$ is shaped in order to satisfy the following inequality
\begin{lemma}\label{lem:explbonus.inequality}
        Assume that $\SP{h^*} \leq c$ and consider the MDP $\wh{M}_k$. For all $T \geq 1$, with probability at least $1-\frac{\delta}{15 t_k^6}$, for any $k \geq 1$, for any $s \in \calS $ we have:
\[
                \max_{a \in \A} \big\{ \wb{r}_k(s,a) + b_{k}(s,a) + \wh{p}_k(\cdot|s,a)^\intercal h^* \big\} \geq \max_{a \in \A} \left\{ {r}(s,a) + {p}(\cdot|s,a)^\intercal h^* \right\}
%                 \left| \wb{r}_k(s,a) - r(s,a) + \left( \wh{p}_k(\cdot|s,a) - p(\cdot|s,a) \right)^\transp h^* \right|
\]
\end{lemma}
Hoeffding's inequality implies that with probability at least $1-\frac{\delta}{15 t_k^6}$, for all pairs $(s,a) \in \mathcal{S}\times \mathcal{A}$, $ \left|\wo{r}_k(s,a) - r(s,a)\right| \leq \beta_{r,k}^{sa}$ and $\left|\left(\wo{p}_k(\cdot|s,a) - p(\cdot|s,a)\right)^\intercal h^*\right| \leq c \;\beta_{p,k}^{sa}$.
Moreover, by definition, with probability 1, $\left|\wo{r}_k(s,a) - r(s,a)\right| \leq \rmaxbound$ and $\left|\left(\wo{p}_k(\cdot|s,a) - p(\cdot|s,a)\right)^\intercal h^*\right| \leq 2 c $.
Finally, we also need to take into account the small bias introduced by $\wh{p}_k(\cdot|s,a)$ compared to $\wo{p}_k(\cdot|s,a)$. By defintion, this bias is not bigger than ${c}/{(N_k(s,a)+1)}$.
In conclusion, the exploration bonus we need to verify Lem.~\ref{eq:exploration.bonus} is
\begin{align}\label{eq:exploration.bonus}
\begin{split}
b_k(s,a) := c \; &\min\left\{\beta_{p,k}^{sa}+ \frac{1}{N_k(s,a)+1} ; 2 \right\}
+ \min \left\{\beta_{r,k}^{sa}; \rmaxbound \right\}
\end{split}
\end{align}
\begin{lemma}\label{L:optimism}
       $\forall k>0$, with probability at least $1-\frac{\delta}{15 t_k^6}$, $\wh{g}^+_k \geq g^*$.
\end{lemma}
\paragraph{Remark.} The exploration bonus quantifies by how much $\wh{L}^+ h^*$ is bigger than $L{h^*} $ and approximately scales as $b_k(s,a) \sim \max\{\rmaxbound,c\}/\sqrt{N_k(s,a)}$. 
In contrast, \ucrl and \scal use an optimistic Bellman operator $\wt{L}$ such that $\wt{L}h^*$ is bigger than $Lh^*$ by respectively $\rmaxbound D\sqrt{\Gamma/N_k(s,a)}$ (\ucrl\footnote{The original bound of \citet{Jaksch10} has $\sqrt{S}$ instead of $\sqrt{\Gamma}$ but $\sqrt{\Gamma}$ can be easily achieved by replacing Hoeffding's inequality by empirical Bernstein's inequality for transition probabilities.}) and $\max\{\rmaxbound,c\}\sqrt{\Gamma/N_k(s,a)}$ (\scal). 
In other words, the optimism in \bonusscal is tighter by a multiplicative factor $\sqrt{\Gamma}$. 
This improvement is achieved by relying on a different argument to prove optimism (Prop.~\ref{prop:bound.gain} instead of a set of plausible MDPs containing the true MDP).
Note that we could extend this approach to \scal in order to save $\sqrt{\Gamma}$. This would require to slightly modify the optimal Bellman operator of Extended Value Iteration (EVI).
More precisely, the Linear Programming problem used in each pair $(s,a)$ to compute the optimistic transition probability $\wt{p}_k(\cdot|s,a)$ should take into account the additional linear constraints $-c\beta_{p,k}^{sa} \leq \left(\wo{p}_k(\cdot|s,a) - \wt{p}_k(\cdot|s,a)\right)^\intercal v \leq c \beta_{p,k}^{sa}$. Extending the result to \ucrl is more challenging since the fact that $\SP{v_n} \leq D$ at every iteration $n$ of EVI also relies on the fact that the extended MDP contains the true MDP. We keep this open question for future work.

\subsection{Other requirements for \scopt}
{\color{red} TODO: move stuff from section 3.2}

\subsection{Regret Analysis of \bonusscal}
\label{app:regret.bonusscal}
{\color{red} TODO: present more the positive side and clarify the proof sketch. Mention work of Shipra and Azar.}

We now give the main result of this section:
% The regret of \bonusscal can be bounded as follows:
\begin{theorem}\label{thm:regret.bonusscal}
 For any \emph{weakly communicating} MDP $M$ such that $\SP{h^{*}_M}\leq c$, with probability at least $1-\delta$ it holds that for any $T\geq 1$, the regret of \bonusscal is bounded as
 \begin{align*}
         \Delta(\bonusscal,T) = O \left( \max \lbrace \rmaxbound, c \rbrace \left( \sqrt{\nextstates S A T \ln \left( \frac{T}{\delta} \right)} + S^2A\ln^2\left(\frac{T}{\delta} \right) \right) \right).
 \end{align*}
\end{theorem}

Given the fact that the optimism in \bonusscal is tighter than in \scal by a factor $\sqrt{\Gamma}$, one might have expected to get a regret bound scaling as $c \sqrt{SAT}$ instead of $c \sqrt{S\Gamma AT}$, thus matching the lower bound of \citet{Jaksch10} as for the dependency in $S$.\footnote{From an algorithmic perspective we achieve the optimal dependence on $S$, although this is not reflecting in the regret bound.}
Unfortunately, such a bound seems difficult to achieve with \bonusscal (and even \scal). While bounding the regret, we have to make appear the difference $(\wh{p}_k(\cdot|s,a) - p(\cdot|s,a))^\transp \wh{h}^+_k$ where $\wh{h}_k^+$ is the (approximate) solution of the optimality equation $\wh{T}_c^+ \wh{h}_k^+ = \wh{h}_k^+ + \wh{g}_k^+ e$. Since $\wh{h}_k^+$ depends on $\wh{p}_k(\cdot|s,a)$, we cannot apply Hoeffding's inequality as in Sec.~\ref{sec:exploration_bonus}. Instead, we have to bound separetely $\|\wh{p}_k(\cdot|s,a) - p(\cdot|s,a))\|_1 \lesssim \sqrt{\Gamma /N_k(s,a)}$ and $ \SP{ \wh{h}^+_k}\leq c$ which will introduce a $\sqrt{\Gamma}$ factor. It is worth pointing out that $\Gamma$ only appears due to statistical fluctuations that we cannot control, and not from the optimism (\ie exploration bonus) that is explicitly encoded in the algorithm. Although the bound is not better than \scal, we can expect some empirical improvement due to the tighter optimism for large $\Gamma$.


Unlike \scal, \bonusscal does not have a regret scaling with $\min\{\rmaxbound D, c\}$ implying that whenever $c> D$, \bonusscal performs worse than \ucrl. \scal builds an extended MDP that contains the true MDP and therefore the shortest path in the extended MDP is shorter than the shortest path in the true MDP implying that $\SP{\wt{h}_k} \leq \rmaxbound D$ (Theorem 4 of \citet{Bartlett2009regal}). It is not clear how to bound $ \SP{ \wh{h}^+_k}$ other than using the prior knowledge $c$. This open question seems a lot related to the one of Sec.~\ref{sec:exploration_bonus} (\ie how to have a tighter optimism in \ucrl) and we also keep it for future work.


\textbf{Proof sketch.} We now provide a sketch of the main steps of the proof of Thm.~\ref{thm:regret.bonusscal} (the full proof is reported in App.~\ref{app:regret.bonusscal}). In order to preserve readability, in the following, all inequalities should be interpreted up to minor approximations and in high probability.
%
% Let $\Delta_k := \sum_{s,a}\nu_k(s,a)(g^* -r(s,a))$ be the regret incurred in episode $k$, where $\nu_k(s,a)$ is the number of visits to $s,a$ in episode $k$. 
Let $\nu_k(s)$ be the number of visits in $s$ during episode $k$ ($\nu_k(s) = \sum_{\A} \nu_k(s,a)$) and $m$ be the total number of episodes. 
By using the optimism proved in Sec.~\ref{sec:exploration_bonus}, we can decompose the regret as:
%
\begin{align*}
\Delta(\bonusscal, T) 
% \lesssim \sum_{k=1}^m \Delta_k 
\lesssim \sum_{k=1}^m \sum_{s} \nu_k(s) \left( \wh{g}^*_k - \sum_{a} r(s,a) \wt{\pi}_k(s,a) \right)
\end{align*}
%
At this point, we would like to lower bound $r(s,a)$ by using Lem.~\ref{lem:explbonus.inequality} and make the solution computed by \scopt (\ie $v_n$) appear.
Lem.~\ref{lem:explbonus.inequality} cannot be used in this scenario since it does not hold for any vector $v_n \in \mathbb{R}^S$.
By using a union bound argument, we define a different exploration bonus $d_k(s,a)$ scaling with an additional $\sqrt{\Gamma}$ factor in the terms $\beta_{p,k}^{Ia}$ (see Lem.~\ref{L:bonus.inequality} in App.~\ref{app:finite}).
This is the reason why we are unable to prove a tighter regret bound than the one of \scal.
By using an analogous of Lem.~\ref{lem:explbonus.inequality} for $d_k$, the fact that $\wb{r}_k = \wh{r}_k - b_k$ and the stopping condition of \scopt, we can write that
%
\begin{align*}
\Delta(\bonusscal, T)
\lesssim &\sum_{k=1}^m \bm{\nu}_k^\intercal(\bm{P}_k-I)\bm{w}_k + \underbrace{
        \sum_{k=1}^m \sum_{s,a} \nu_k(s) \wt{\pi}_k(s,a) \Big( b_k(s,a) + d_k(s,a) \Big)
}_{\wt{\Delta}(b_k,d_k)}
\end{align*}
%
$w_k$ is obtained by ``recentering'' $v_n$ around $0$ so that $\|w_k\|_\infty = \SP{w_k}/2 \leq c/2$, $\bm{\nu}_k := (\nu_k(s))_{s \in \calS} $ and  $\bm{P}_k:=\left(\sum_{a}p(s'|s,a)\widetilde{\pi}_{k}(s,a)\right)_{s,s'\in \mathcal{S}}$.
The proof follows by noticing that $d_k(s,a) + b_k(s,a) \leq 2 d_k(s,a)$, thus all the remaining terms can be bounded as in~\citep{fruit2018constrained}.
In particular, the dominant terms in $\wt{\Delta}(d_k,d_k)$ (and in the overall regret) are $\sum_k \nu_k(s,a) \beta_{r,k}^{sa}$ and $\sum_k \nu_k(s,a) \beta_{p,k}^{sa}$ that are of order $\wt{O}(\rmaxbound\sqrt{SAT})$ and $\wt{O}(c\sqrt{\Gamma S A T}+cS^2A)$, respectively.
Note that the proof of the regret is simpler than the one of other OFU approaches since the exploration bonus encodes all the deviation between the estimated MDP at episode $k$ and the true one.



==> backup20180923/sec_conclusion.tex <==
% !TEX root = main.tex
\section{Conclusion}
We provided the first analysis of exploration bonus in infinite-horizon undiscounted problems, a more challenging setting than the finite-horizon~\citep[see \eg][]{pmlr-v70-azar17a,kakade2018variance,qlearning2018}.
Compared to the finite-horizon case, we also extended the analysis to the continuous case and we provided the first implementable and efficient (no need to plan on an extend MDP) algorithm.
We finally showed, through a formal derivation of the exploration bonus, that the empirical count-based exploration bonuses are in general not sufficient to provide optimism and thus prone to under-exploration. In particular, the knowledge of the span of the optimal bias function is required in order to properly scale the bonus.
% For this reason, we believe that it will not be easy or even possible to derive a bonus variant of \ucrl (in fact we leveraged the \scal setting).
Moreover, even in the finite-horizon case, the mentioned approaches use the knowledge of the horizon to scale the bonus. The planning horizon is in turn an upper-bound to the span of the optimial value function, thus they exploit the same prior knowledge required by \bonusscal and \scalcont.

Finally, we proved the tightest level of optimism for OFU algorithms by achieving the optimal dependence in the bonus \wrt the state dimensionality (it cannot further reduced while preserving theoretical guarantees). Unfortunately, this tighter optimism does not implies a tighter bound leaving open the quest for closing the gap between lower and upper bound in infinite-horizon undiscounted settings.
Moreover, it is unclear to us if the exploration bonus can be extended to settings where no-prior knowledge of the span of the optimal bias function is available, \eg in communicating (see \ucrl~\citep{Jaksch10}) or weakly-communicating MDPs (see \tucrl~\citep{fruit2018truncated}). We leave this question for future work.



==> backup20180923/sec_continuous.tex <==
% !TEX root = main.tex
\section{\scalcont: \bonusscal for continuous state space}
\label{S:exploration.bonus.continuous}
We now consider an MDP with continuous state space $\calS = [0,1]$ and discrete action space $\A$.
In general, it is impossible to approximate an arbitrary function with only a finite number of samples. As a result, without further assumptions on the reward and transition kernel of the MDP, the problem is not learnable. We therefore make the same smoothness assumption as \citet{DBLP:journals/corr/abs-1302-2550} (H\"older continuity):
% We make the natural assumption of smoothness of the reward and transition function (see~\citep{DBLP:journals/corr/abs-1302-2550}).
\begin{assumption}\label{asm:continuous.mdp}
There exist $L, \alpha > 0$ s.t. for any two states $s,s' \in \calS$ and any action $a\in \A$:
\begin{equation*}
 |r(s,a) - r(s',a)| \leq \rmaxbound L |s -s'|^{\alpha} ~~~ \text{ and } ~~~ \|p(\cdot|s,a) - p(\cdot|s',a)\|_1 \leq L |s-s'|^{\alpha}
\end{equation*}
%         \begin{enumerate}[label=(\alph*)]
%                 \item $|r(s,a) - r(s',a)| \leq \rmaxbound L |s -s'|^{\alpha}$
%                 \item $\|p(\cdot|s,a) - p(\cdot|s',a)\|_1 \leq L |s-s'|^{\alpha}$
%         \end{enumerate}
\end{assumption}
In order to apply \bonusscal to a continuous problem, a natural idea is to discretize the state space as is done by \citet{DBLP:journals/corr/abs-1302-2550}.
We therefore partition $\calS$ into $S$ intervals defined as $I_1 := [0, \frac{1}{S}]$ and $I_k = (\frac{k-1}{S}, \frac{k}{S}]$ for $k=2,\ldots, S$.
The set of \emph{``aggregated''} states is then $\mathcal{I} := \{I_1, \ldots, I_S\}$ ($|\mathcal{I}| = S$). As expected, the number of intervals $S$ will play a central role in the regret.
Note that the terms $N_k(s,a,s')$ and $N_k(s,a)$ defined in Sec.~\ref{S:exploration.bonus} are still well-defined for $s$ and $s'$ lying in $[0,1]$ but are $0$ except for a finite number of $s$ and $s'$ (see Def.~\ref{def:estimated.cont.mdp}).
For any subset $I\subseteq \mathcal{S}$, the sum $\sum_{s \in I} u_{s} $ is also well-defined as long as the collection $\left(u_{s} \right)_{s \in I}$ contains only a finite number of non-zero elements. We can therefore define the \emph{aggregated} counts, rewards and transition probabilities for all $I,J \in \mathcal{I}$ as: $N_k(I,a) := \sum_{s \in I} N_k(s,a)$, 
% 
\begin{align*}
% N_k(I,a)&:= \sum_{s \in I} N_k(s,a),\\
% \wo{p}_k(s'|s,a) := \frac{N_k(s,a,s')}{N_k(s,a)}  ~~\text{ and }~~  \wo{r}_k(s,a) := \frac{1}{N_k(s,a)} \sum_{t=1}^{t_k -1} r_t(s_t,a_t) \mathbbm{1}(s_t,a_t = s,a)
% 
\wb{r}^{ag}_k(I,a) := \frac{1}{N_k(s,a)} \sum_{t=1}^{t_k -1} r_t(s_t,a_t) \mathbbm{1}(s_t \in I,a_t = a), ~~
\wb{p}^{ag}_k(J|I, a) := \frac{\sum_{s' \in J} \sum_{s \in I} N_k(s,a,s')}{\sum_{s \in I} N_k(s,a)}.
% \frac{\sum_{s'\in J} \sum_{s \in I} N_k(s,a,s')}{N_k(I,a)}
%         &\wb{r}^{ag}_k(I,a):= \frac{1}{N_k(I,a)} \sum_{t=1}^{t_k-1} r_t(s_t,a_t) \mathbbm{1}(s_t \in I(s), a_t=a)\\
%         &\wb{p}^{ag}_k(J|I, a) := \frac{\sum_{s'\in J} \sum_{s \in I} N_k(s,a,s')}{N_k(I,a)}
\end{align*}
Similarly to the discrete case, we define the exploration bonus of an aggregated state as
\begin{align}\label{eq:exploration.bonus.cont}
\begin{split}
        b_k(I,a) := &c \; \min\left\{\beta_{p,k}^{Ia}+ \frac{1}{N_k(I,a)+1} ; 2 \right\}
                            + \min \left\{\beta_{r,k}^{Ia}; \rmaxbound \right\} + (c+\rmaxbound)L S^{-\alpha}
\end{split}
\end{align}
%
% and pick an arbitrary reference aggregated state $\wb{I}$. 
While $\beta_{p,k}^{Ia}$ and $\beta_{r,k}^{Ia}$ are defined as in~\eqref{eq:confidence.intervals} on the discrete ``aggregated'' MDP, the main difference with the discrete bonus~\eqref{eq:exploration.bonus} is an additional $O(cLS^{-\alpha})$ term that accounts for the fact that the states that we aggregate are not completely identical but have parameters that differ by at most $LS^{-\alpha}$. 
We pick an arbitrary reference aggregated state $\wb{I}$ and define $\wh{M}^{ag}_k = (\mathcal{I}, \A, \wh{p}_k^{ag}, \wh{r}_k^{ag})$ the ``aggregated'' (discrete) analogue of $\wh{M}_k$ defined in Sec.~\ref{S:exploration.bonus}, where $\wh{r}_k = \wb{r}^{ag}_k + b_k$ and
\[
        \wh{p}^{ag}_k(J|I,a) = \frac{N_k(I,a) \wb{p}^{ag}_k(J|I,a)}{N_k(I,a) + 1} + \frac{\mathbbm{1}(J=\wb{I})}{N_k(I,a) + 1},
\]
Similarly we ``augment'' $\wh{M}^{ag}_k$ into $\wh{M}^{ag+}_k = (\mathcal{I}, \A^+, \wh{p}^{ag+}_k, \wh{r}^{ag+}_k)$ (analogue of $\wh{M}_k^+$ in Sec.~\ref{S:exploration.bonus}) by duplicating each transition in $\wh{M}^{ag}_k$ with the transition probability unchanged and the reward set to $0$.

% \scalcont applies the same idea as \bonusscal with $\wh{M}^+_k$ replaced by $\wh{M}^{ag+}_k$.
At each episode $k$, \scalcont uses \scopt (with the same parameters as in Sec.~\ref{S:exploration.bonus}) to solve optimization problem \eqref{eq:opt.superior.spanc} on $\wh{M}^{ag+}_k$.
% \begin{equation}\label{eq:scalc.optimization}
%         \max_{\pi \in \PiC(\wh{M}^{ag+}_k)} g^{\pi}_{\wh{M}^{ag+}_k}
% \end{equation}
This is possible because although the state space of $M^*$ is infinite, $\wh{M}^{ag+}_k$ has only $S < +\infty$ states.
% Note that the optimization is performed directly in the finite aggregated space, thus can be efficiently carried out despite $M^*$ being continuous.
\scopt returns an \emph{optimistic} (nearly) optimal policy $\wt{\pi}_k$ 
% ($g^{\wt{\pi}_k}(\wh{M}^{ag+}_k) \geq g^*_{M^*} - \epsilon_k$) 
satisfying the span constraint.
This policy is defined in the aggregated discrete state space but can easily be extended to the continuous case since as $\wt{\pi}_k(s,a) = \wt{\pi}_k(I(s),a)$ for any $(s,a)$.
Policy $\wt{\pi}_k$ is executed until the end of the episode (see Alg.~\ref{fig:ucrl.constrained}).


\subsection{Regret Analysis of \scalcont}
% As mentioned in Sec.~\ref{sec:exploration_bonus}, the key point in the regret analysis is to prove that $\wt{\pi}_k$ is (approximately) gain optimistic.
Before to state the regret of $\scalcont$ we provide a sketch of the proof of optimism (as done for the discrete case).
To be able to compare the solution of optimisation~\eqref{eq:opt.superior.spanc} on $\wh{M}^{ag+}_k$ (discrete state space MDP) with the solution of~\eqref{eq:opt.superior.spanc} on $M^*$ (continuous state space MDP), we define the continuous state space MDP $\wh{M}_k$ as follows:
% \scalcont directly operates in the discrete state space $\mathcal{I}$. 
% We can clearly see the aggregated MDP $\wh{M}^{ag+}_k$ as induced by an estimated MDP $\wh{M}_k$ in the continuous state space.
% Since there exists infinitely many continuous MDP inducing the aggregated one, we decided to define $\wh{M}_k$ as follows.
\begin{definition}[Estimated continuous MDP]\label{def:estimated.cont.mdp}
        Let $\wh{M}_k = (\calS,\A, \wh{p}_k, \wh{r}_k)$ be the continuous state space MDP \st for all $(s,a) \in \calS \times \A$,
        $\wh{r}_k(s,a) = \wb{r}_k^{ag}(I(s), a) + b_k(I(s),a)$ and\footnote{The function $I : \calS \to \mathcal{I}$ maps a state $s$ to the interval containing $s$.} 
                \[
                        \wh{p}_k(s'|s,a) = \frac{N_k(I(s),a) \wb{p}_k(s'|s,a)}{N_k(I(s),a)+1} + \frac{S \cdot \mathbbm{1}(s' \in I(\wb{s}))}{N_k(I(s),a) + 1}.
                \]
                where the term $\wb{p}_k(s'|s,a)$ is the Radon-Nikodym derivative of the cumulative density function $F(s) = \sum_{s' \leq s} \frac{\sum_{x \in I(s)}N_k(x,a,s')}{N_k(I(s),a)}$, meaning that for any measurable function $f$ and any measurable set $Z \subseteq [0,1]$, $\int_Z \wb{p}_k(s'|s,a) f(s') \mathrm{d}s' = \sum_{s' \in Z} \frac{\sum_{x \in I(s)}N_k(x,a,s')}{\sum_{x \in I(s)}N_k(x,a)} f(s')$.
\end{definition}
By definition, $\forall J \in \mathcal{I}$, $\int_{J} \wb{p}_k(s'|s,a) \mathrm{d}s' = \wb{p}_k^{ag}(J|s,a) := \wb{p}_k^{ag}(J|I(s),a)$ and $\forall (s,J) \in \calS \times \mathcal{I}$:
\begin{equation}\label{eq:integral.p.perturbed}
        \begin{aligned}
                \int_{J} \wh{p}_k(s'|s,a) \mathrm{d}s'
                &= \int_{J} \frac{N_k(I(s),a) \wb{p}_k(s'|s,a)}{N_k(I(s),a)+1} \mathrm{d}s' + 
                    \frac{
                    S \int_J \mathbbm{1}(s' \in I(\wb{s}))\mathrm{d}s'
                    }{N_k(I(s),a) + 1}
                = \wh{p}_k^{ag}(J|I(s),a)
        \end{aligned}
\end{equation}
%
It is possible to prove an analogue of Lem.~\ref{lem:explbonus.inequality} for the continuous MDPs $\wh{M}_k$ and $M^*$.
% Similarly to the discrete case, the exploration bonus is defined in order to satisfy (an analogue of) Lem.~\ref{lem:explbonus.inequality} for the continuous MDPs $\wh{M}_k$ and $M^*$.
% The derivation of the bonus follows the same idea. 
% The main and crucial difference in the proof is the ``aggregation'' of samples to build the estimates $\wb{p}_k$ and $\wb{r}_k$.
The main and crucial difference in the proof is that due to the aggregation of states, $\wb{p}_k$ and $\wb{r}_k$ do not statistically concentrate around the true values $p$ and $r$. To overcome this problem we decompose $\wh{p}_k -p$ into the sum of three terms $(\wh{p}_k -\wo{p}_k) + (\wo{p}_k - \wt{p}_k) +  (\wt{p}_k -p)$ with $\wt{p}_k(s'|s,a) :=\frac{1}{N_k(I(s),a)}\sum_{x \in I(s)} N_k(x,a) p(s'|x,a)$. We show that $\int_{\calS}(\wt{p}_k(s') -p(s'))h^*(s')\mathrm{d}s' = O(LS^{-\alpha})$ (Asm.~\ref{asm:continuous.mdp}: smoothness assumption) while $\int_{\calS}(\wh{p}_k(s') -\wo{p}_k(s')) h^*(s')\mathrm{d}s' = O(1/N_k)$ (biased estimator). 
The term $\int_{\calS}(\wo{p}_k(s') - \wt{p}_k(s')) h^*(s')\mathrm{d}s'$ can be bounded using concentration inequalities but requires more work than in the discrete case. In the discrete case, for a given state-action pair $(s,a) \in \calS \times \A$, the difference $(\wo{p}_k(\cdot|s,a) -\wt{p}_k(\cdot|s,a))^\intercal h^*$ is usually interpreted as the deviation of a sum of independent random variables from its expectation \citep[Section 4.4]{bandittorcsaba} and can be bounded using Hoeffding's inequality. 
Since there is only a finite number of possible $(s,a)$, it is possible to take a union bound over state-action pairs. In the continuous case, the difference $\int_{\calS}(\wo{p}_k(s') - \wt{p}_k(s')) h^*(s')\mathrm{d}s'$ does not just depend on a single $s$ but on the (random) set of states belonging to a given interval $I \in \mathcal{I}$ that have been visited. 
There is an uncountable number of possible such sequences of states and so we can not use a union bound argument. 
Instead, we rely on a martingale argument and Azuma inequality for the proof. We decompose $\wh{r}_k -r$ as $(\wh{r}_k -\wt{r}_k) + (\wt{r}_k -r)$ with $\wt{r}_k(s,a) := \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a) r(x,a)$ and proceed similarly for the reward.
% to which $\wb{p}_k$ and $\wb{r}_k$ statistically concentrate.\footnote{We define $\wt{r}_k(s,a) := \frac{1}{N_k(I(s),a)} \sum_{x \in I(s)} N_k(x,a) r(x,a)$ and $\wt{p}_k(s'|s,a) :=\frac{1}{N_k(I(s),a)}\sum_{x \in I(s)} N_k(x,a) p(s'|x,a)$. }
% We thus decompose $\wh{p}_k -p$ as $(\wh{p}_k -\wo{p}_k) + (\wo{p}_k - \wt{p}_k) +  (\wt{p}_k -p)$ and bound separately all the differences. Similarly, we decompose $\wh{r}_k -r$ as $(\wh{r}_k -\wt{r}_k) + (\wt{r}_k -r)$.
% Due to the aggregation, the samples used to construct $\wb{p}_k$ and $\wb{r}_k$ are neither independent nor identically distributed. We thus rely on Azuma's inequality for martingale difference sequence in order to show that $|(\wb{p}_k(\cdot|s,a) - \wt{p}_k(\cdot|s,a))^\transp h^*| \leq c \beta_{p,k}^{I(s)a}$ and $|\wb{r}_k(s,a) - \wt{r}_k(s,a)| \leq \beta_{r,k}^{I(s)a}$.\footnote{With an abuse of notation, we define $p(\cdot|s,a)^\transp v := \int_{\calS} p(s'|s,a) v(s') \mathrm{d}s'$ for continuous MDPs.}
% As a consequence of the decomposition through $\wt{p}_k$ and $\wt{r}_k$, we are left with an additional term compared to the discrete case. This term is directly bounded by using the smoothness (Asm.~\ref{asm:continuous.mdp}) of the true MDP $M^*$, leading to $|(\wt{p}_k(\cdot|s,a) - p(\cdot|s,a))^\transp h^*| \leq c L S^{-\alpha}$ and $|\wt{r}_k(s,a) - r(s,a)| \leq \rmaxbound LS^{-\alpha}$.
% Clearly, the bonus contains also the term due to the perturbation of $\wh{p}_k$ \wrt to $\wb{p}_k$, as in the discrete case.
The detailed proof can be found in App.~\ref{app:continuous} (Lem.~\ref{L:bonus.inequality.continuous}).

Concerning optimism, an analogous of Lem.~\ref{L:optimism} can be proved for the continuous case. In particular, the same argument used for the discrete case (an analogous of Lem.~\ref{lem:explbonus.inequality} together with Prop.~\ref{prop:bound.gain}) is sufficient to prove that the exploration bonus in~\eqref{eq:exploration.bonus.cont} makes $\wh{M}_k$ optimistic \wrt $M^*$: $g^*_c(\wh{M}_k) \geq g^*$.
The key step in the continuous case is to relate the gain of the discrete MDP $\wh{M}^{ag+}_k$ to the one of $\wh{M}_k$.
We start noticing that, starting from a value $v_0(s) = 0$ ($\forall s$), the application of the Bellman operator of $\wh{M}^{ag}_k$ and $\wh{M}_k$ is such that $\wh{L}^{ag} v_n(s) = \wh{L}v_n(s)$, $\forall s \in \calS, n >0$.
This is due to the fact that $v_n$ is constant over any interval $I$ and~\eqref{eq:integral.p.perturbed} holds. 
Then, $\forall n,s,~\wh{T}_c^{ag} v_n(s) = \wh{T}_c v_n(s)$ implying $g^*_c(\wh{M}^{ag}_k) = g^*_c(\wh{M}_k)$.
The optimism of $\wh{M}^{ag+}_k$ follows by the fact that the ``augmentation'' does not impact the gain: $g^*_c(\wh{M}^{ag+}_k) = g^*_c(\wh{M}^{ag}_k)$~\citep[][Lem. 20]{fruit2018constrained}.
The detailed proof can be found in App.~\ref{app:continuous} (Lem.~\ref{L:optimism.cont}).


We are now ready to state the regret bound for $\scalcont$.
\begin{theorem}\label{thm:regret.scalcont}
        For any continuous MDP $M$ with state space $\calS \in [0,1]$ and $A$ actions such that $\SP{h^*_M} \leq c$, with probability at least $1 - \delta$ it holds that for any $T \geq 1$, the regret of \scalcont is bounded as
        \[
                \Delta(\scalcont,T) = O
                \left( \max{\left\lbrace \rmaxbound,c \right\rbrace} \left( S\sqrt{A T \ln\left(\frac{T}{\delta}\right)}
                        + S^2A\ln^2\left(\frac{T}{\delta} \right) 
        + L S^{-\alpha}T \right) \right)
        \]
        For $T \geq L^{\sfrac{2}{\alpha}} A$ and by setting $S = \left(\alpha L \sqrt{\frac{T}{A}}\right)^{\sfrac{1}{(\alpha + 1)}}$, the regret is bounded as
        \[
                \Delta(\scalcont,T) = \wt{O} \left(\max\{c,\rmaxbound\} L^{\sfrac{1}{(\alpha+1)}} A^{\sfrac{\alpha}{(2\alpha+2)}} T^{\sfrac{(\alpha+2)}{(2\alpha+2)}} 
%                \sqrt{\ln\left(\frac{T}{\delta} \right)} 
\right) 
        \]
\end{theorem}
Thm.~\ref{thm:regret.scalcont} shows that \scalcont achieves the same regret of \uccrl~\citep{DBLP:journals/corr/abs-1302-2550} while being more computationally efficient.
Furthermore, we notice that, as mentioned by~\citep{DBLP:journals/corr/abs-1302-2550}, the analysis can be extended tot the $d$-dimensional case leading to a regret of $\wt{O}(T^{\sfrac{(2d+\alpha)}{(2d+2\alpha)}})$.

Finally, \scalcont can be extended to the settings considered by~\citep{pmlr-v37-lakshmanan15}
If we additionally assume that the transition function is $\kappa$-times smoothly differentiable, it is possible to prove that a variant of \scalcont using kernel density estimation for the transition function will achieve a regret bound of $\wt{O}(T^{\sfrac{(\beta + \alpha\beta+2\alpha)}{(\beta + 2\alpha\beta+2\alpha)}})$ where $\beta := \kappa + \alpha$.
In the case of Lipschitz model, \ie $\alpha=1$, this means that it is possible obtain an asymptotic regret (as $\kappa \to \infty$) of $\wt{O}(T^{2/3})$ while \scalcont is achieving $\wt{O}(T^{3/4})$.
\todom{to check the paper in order to see if there are major problems in extending the analysis}



==> backup20180923/sec_experiments.tex <==
% !TEX root = main.tex
\section{Experiments}\label{sec:experiments}

For the experiments we consider a tighter concentration inequality for the reward: empirical Bernstein's inequality~\citep{audibert2007tuning,Maurer2009empirical}. This does not affect the regret guarantees but slightly improves the empirical regret at the expense of a negligible additional computational cost. The bonus is then defined using:
\begin{align*}
\beta_{r,k}^{sa}:=
         \sqrt{\frac{14 
                         \wh{\sigma}_{r,k}^2(s,a)
                        b_{k,\delta}
                }{\max\lbrace 1, N_k(s,a)\rbrace}} + \frac{\frac{49}{3}
\rmaxbound
        b_{k,\delta}
        }{\max\lbrace 1, N_k(s,a)-1 \rbrace},\\
\end{align*}
where $\wh{\sigma}_{r,k}^2(s,a)$ is the empirical variance of $r(s,a)$.
Although tighter, this new confidence bound might be of limited practical interest for high dimensional problems as computing $\wh{\sigma}_{r,k}^2(s,a)$ can be computationally expensive.


==> backup20180923/sec_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
While learning in an unknown environment, a reinforcement learning (RL) agent must trade off the \textit{exploration} needed to collect information about the dynamics and reward, and the \textit{exploitation} of the experience gathered so far to gain as much reward as possible. 
In this paper, we focus on the regret framework in \emph{infinite-horizon average-reward} problems~\citep{Jaksch10}, where the exploration-exploitation performance is evaluated by comparing the rewards accumulated by the learning agent and an optimal policy.
\citet{Jaksch10} showed that it is possible to efficiently solve the exploration-exploitation dilemma using the \emph{optimism in face of uncertainty} (OFU) principle.
OFU methods build confidence intervals on the dynamics and reward (\ie construct a set of plausible MDPs), and execute the optimal policy of the ``best'' MDP in the confidence region~\citep[\eg][]{Bartlett2009regal,DBLP:journals/corr/abs-1302-2550,fruit2017optionsnoprior,fruit2018constrained}.
Since, with high probability, the true MDP is contained in the set of plausible MDPs, the recovered policy is, in average-reward, better than the true one, \ie \emph{optimistic}. This property is fundamental to derive regret guarantees.

% \textbf{Set of plausible MDPs vs. empirical estimate.} 
Extended Value Iteration~\citep{Jaksch10} allows to efficiently plan over the set of plausible MDPs but its computational cost can quickly become prohibitive in large MDPs.
% Despite the planning over the set of plausible MDPs can be efficient solved with Extended Value Iteration~\citep{Jaksch10}, its computational cost can quickly become prohibitive in large MDPs.
EVI is a variant of Value Iteration (VI)~\citep{puterman1994markov} that requires to solve an additional linear programming problem at each iteration and for each state-action pair in order to select the ``best'' transition function in the confidence set.
The computational cost of this operation is linear in the number of states $S$.
To overcome this limitation, we would like to apply directly VI on the estimated MDPs. 
Unfortunately, this na\"{i}ve approach leads to under-exploration since there is no more explicit incentive to visit unexplored regions (thus optimism is lost).


In this paper, we will show that efficient planning (\ie on the empirical MDP) and optimism can be obtained by means of an exploration bonus.
The exploration bonus boosts the reward of state-action pairs that are poorly visited, thus enforcing exploration.
This approach has been widely employed for exploration in deep reinforcement learning~\citep[\eg][]{Bellemare:2016aa,tang2017exploration,ostrovski2017count-based,MartinSEH17} (with the name of \emph{count-based exploration}) and only formally analysed in the finite horizon setting \citep{pmlr-v70-azar17a,kakade2018variance,qlearning2018}. Unfortunately it is difficult to find examples of RL tasks with an intrinsic horizon known to the learning agent. For this reason, the infinite horizon setting is often better suited to model an RL problem. 
We will show that the empirical bonus used by count-based approaches is not sufficient to guarantee sublinear regret.
In particular, the knowledge of  an upper bound $c$ on the span of the optimal bias function is necessary in order to properly scale the exploration bonus.
Let $N_k(s,a)$ be the number of observation of a state-action pair, we will show that a bonus of order $\wt{O}\left(c \sqrt{\frac{1}{N_k(s,a)}}\right)$ is sufficient to guarantee optimism.
Compared to standard approaches (\eg \ucrl~\citep{Jaksch10} and \scal~\citep{fruit2018constrained}), the proposed bonus allows to achieve a tighter optimism by a $\sqrt{S}$-factor.
As a consequence, the proposed algorithm are less prone to over-exploration and, algorithmically, they achieve the best dependence \wrt the state dimension.
This improvement is not reflected in the final regret bound with the current statistical analysis. It is an open question whether the analysis could be improved or if it is an intrinsic limitation of online RL. 
% This improvement is not reflected in the theoretical analysis due to statistical limitations in the current proof technique.
%Moreover, we show that the level of optimism used by several OFU approach (\eg \scal~\citep{fruit2018constrained}) can be reduced by a factor $\sqrt{S}$, matching the lower bound from an algorithmic perspective.

As a consequence of this analysis, we introduce and analyse \bonusscal, an efficient algorithm for exploration-exploitation in discrete MDPs.
For any discrete MDP with $S$ states, $A$ actions and $\Gamma$ possible next states, \bonusscal achieves a state-of-the-art regret bound of $\wt{O}\left(c \sqrt{\Gamma SAT}\right)$, while being more computationally efficient.
We further extend the analysis to smooth MDPs with continuous state space where the proposed algorithm, \scalcont, is able to achieve the same regret guarantees of \uccrl~\citep{DBLP:journals/corr/abs-1302-2550}.

\todom{I would probably suggest to have a more explicit ``contributions'' paragraph in the intro with even ``informal'' theorem statements. This is quite common at COLT/ALT conferences.}







==> backup20180923/sec_preliminaries.tex <==
% !TEX root = main.tex
\section{Preliminaries}\label{sec:preliminaries}

\subsection{Markov Decision Processes}
This section is devoted to provide the basic concepts about Markov Decision Processes (MDPs) with average-reward criterion.
We consider a \emph{weakly-communicating}\footnote{
In a weakly-communicating MDP, the set $\calS$ can be decomposed into two subsets: a \emph{communicating} set in which for any pair of states $s,s'$ there exists a policy that has a non-zero probability to reach $s'$ starting from $s$, and a set of states that are \emph{transient} under all policies.\textcolor{red}{do we want to mention multi-chain?}}
MDP \citep[Sec. 8.3]{puterman1994markov} $M = ( \calS, \A, p, r )$ with a set of states $\calS$ and a set of actions $\A$.
%While the action space is finite ($|\A|=A$), the state space is considered finite ($|\calS|=S$) is Sec.~\ref{S:exploration.bonus} and continuous in Sec.~\ref{S:exploration.bonus.continuous} ($\calS = [0,1]$).
For sake of clarity, here we consider a finite MDP $M$ but all the stated concepts extend to the case of continuous state space,~\citep[see \eg][]{DBLP:journals/corr/abs-1302-2550}.

Each state-action pair $(s,a)$ is characterized by a reward distribution with mean $r(s,a)$ and support in $[0, \rmaxbound]$ as well as a transition probability distribution $p(\cdot|s,a)$ over next states.
We denote by $S = |\calS|$ and $A = |\A|$ the number of states and action, and by $\nextstates = \max_{s \in \calS, a \in \A} \|p(\cdot|s,a)\|_{0} \leq S$ the maximum support of all transition probabilities $p(\cdot|s,a)$.
A stationary Markov randomized policy $\pi : \calS \rightarrow P(\A)$ maps states to distributions over actions.
The set of stationary randomized (resp. deterministic) policies is denoted by $\SR$ (resp. $\SD$).
Any policy $\pi \in \SR(M)$ has an associated \emph{long-term average reward} (or gain) and a \emph{bias function} defined as
%
\begin{align*}
        g^\pi_M(s) := \lim_{T\to +\infty} \mathbb{E}_{\mathbb{Q}}\Bigg[ \frac{1}{T}\sum_{t=1}^T r(s_t,a_t) \Bigg],~~ 
        h^\pi_M(s) := \underset{T\to +\infty}{C\text{-}\lim}~\mathbb{E}_{\mathbb{Q}}\Bigg[\sum_{t=1}^{T} \big(r(s_t,a_t) - g_M^\pi(s_t)\big)\Bigg],
\end{align*}
where $\mathbb{Q} := \mathbb{P}\left(\cdot|a_t \sim \pi(s_t); s_0=s; M\right)$ and the bias $h^\pi_M(s)$
 measures the expected total difference between the reward and the stationary reward in \emph{Cesaro-limit}\footnote{For policies with an aperiodic chain, the standard limit exists.} (denoted $C\text{-}\lim$). Accordingly, the difference of bias values $h^\pi_M(s)-h^\pi_M(s')$ quantifies the (dis-)advantage of starting in state $s$ rather than $s'$. In the following, we drop the dependency on $M$ whenever clear from the context and denote by $\SP{h^\pi} := \max_s h^\pi(s) - \min_{s} h^\pi(s)$ the \emph{span} of the bias function.
%
In weakly communicating MDPs, any optimal policy $\pi^* \in \argmax_\pi g^\pi(s)$ has \emph{constant} gain, i.e., $g^{\pi^*}(s) = g^*$ for all $s\in\calS$. 
Moreover, there exists a policy $\pi^* \in \argmax_\pi g^\pi(s)$ for which $(g^*,h^*) = (g^{\pi^*},h^{\pi^*})$ satisfy the \emph{optimality equation}
\begin{equation}\label{eq:optimality.equation}
                h^* = L h^* - g^* e, \quad\text{ where }\;\; e = (1,\dots,1)^\intercal.
\end{equation}
where L is the \emph{optimal} Bellman operator: $\forall v \in \Re^S, s\in\calS,$
%
\begin{equation}\label{eq:optimal.bellman.op}
  \begin{aligned}
          Lv(s) &:=
        \max_{a \in \A} \{r(s,a) + p(\cdot|s,a)^\transp v\}
  \end{aligned}
\end{equation}
%
Note that $h^*$ is finite, \ie $\SP{h^*} < +\infty$.
Finally,
    $D := \max_{(s,s') \in \calS\times \calS, s\neq s'} \{\tau_{M}(s \to s')\}$
denotes the diameter of $M$,
where $\tau_{M}(s\to s')$ is the minimal expected number of steps needed to reach $s'$ from $s$ in $M$ (under any policy).

\subsection{Planning under span constraint}\label{sec:scopt}
In this section we introduce and analyse the problem of planning under bias span constraint, \ie by imposing that $\SP{h^\pi_M} \leq c$, for any policy $\pi$.
This problem is at the core of the proposed algorithms (\bonusscal and \scalcont) for exploration-exploitation.
Formally, we define the optimization problem:
\begin{equation}\label{eq:opt.superior.spanc}
        g^*_c(M) := \sup_{\pi \in \PiC(M)}\{g^\pi_M\},
\end{equation}
where $M$ is any MDP (with discrete or continuous state space) \st $\PiC(M) := \{\pi \in \SR : \SP{h^\pi_M} \leq c \wedge \SP{g^\pi_M} = 0\} \neq \emptyset$.
This problem is a slight variation of the bias-span constrained problem considered  by~\citet{Bartlett2009regal,DBLP:journals/corr/abs-1302-2550,pmlr-v37-lakshmanan15}, for which no known-solution is available.
% Since $r$ is bounded, the supremum always exists.
On the other hand, problem~\ref{eq:opt.superior.spanc} has been widely analysed by~\citet{fruit2018constrained}.

Denote by $\Pi^*_c(M)$ the set of maximizers,~\citet[][Lem. 3]{fruit2018constrained} showed that, when the MDP $M$ is unichain, problem~\ref{eq:opt.superior.spanc} is well defined and a maximizer $\pi^*_c \in \Pi^*_c(M) \subseteq \SR$ exists.
Moreover, contrary to the unconstrained gain maximization problem, they proved that there exists an MDP $M$ with no deterministic policy being optimal, \ie $\Pi^*_c(M) \neq \emptyset$ and $\Pi^*_c(M) \cap \SD = \emptyset$~\citep[][Lem. 2]{fruit2018constrained}. For this reason, $\PiC(M)$ is defined on stationary \emph{randomized} (not just deterministic) policies.

Problem~\ref{eq:opt.superior.spanc} can be solved using \scopt~\citep{fruit2018constrained}, a version of (relative) value iteration~\citep{puterman1994markov,bertsekas1995dynamic}, where the optimal Bellman operator is modified to return value functions with span bounded by $c$, and the stopping condition is tailored to return a constrained-greedy policy with near-optimal gain.
%
Given $v \in \Re^{S}$ and $c \geq 0$, we define the value operator $\opT{}:\Re^{S}\rightarrow \Re^{S}$ as
%
        \begin{align}\label{eq:opT}
                \opT{v} = \proj{Lv} = \begin{cases}
                        Lv(s) & \forall s \in \overline{\calS}(c,v)\\
                        c + \min_s \{Lv(s)\} & \forall s \in \mathcal{S} \setminus \overline{\calS}(c,v)
                \end{cases}
        \end{align}
        where $\overline{\calS}(c,v) = \left\{s \in \mathcal{S} | Lv(s) \leq \min_s \{Lv(s)\} + c \right\}$ and $\proj{}$ is a projection operator (see~\citep[][App. D]{fruit2018constrained} for details). 
        In other words, operator $\opT{}$ applies a \emph{span truncation} to the one-step application of $L$, which guarantees that $\SP{\opT{v}} \leq c$. 
Given a vector $v_0\in\Re^S$ and a reference state $\wb s$ \scopt implements relative value iteration where $L$ is replaced by $T_c$:
 %
 $v_{n+1} = \opT{v_{n}} - \opT{v_{n}}(\wb{s})e$.

The convergence of \scopt is guaranteed only under certain conditions: I) The optimal Bellman operator $L$ is a $1$-step $\gamma$-span-contraction~\citep[][Asm. 6]{fruit2018constrained}; II)  operator $\opT{}$ is globally feasible at any vector $v \in \mathbb{R}^S$ such that $\SP{v} \leq c$ \ie for all $s \in \calS,~\min_{s \in \A_s} \{r(s,a) + p(\cdot|s,a)^\transp v \} \leq \min_{s'} \{Lv(s')\} + c$~\citep[][Asm. 9]{fruit2018constrained}. 
%
The fact that $\opT{}$ is globally feasible at $v$ implies that there exists a (stationary randomized) policy $\pi =G_c v$ such that $r_\pi + P_\pi v = T_c v$.\footnote{$G_c$ denotes the greedy operator associated to $\opT{}$~\citep[][Def. 2]{fruit2018constrained}, while $P_\pi \in \mathbb{R}^{\calS \times \calS}$ and $r_\pi \in \mathbb{R}^{\calS}$ are the transition matrix and reward vector associated to a policy $\pi$ .}
Under Asm. 6, \citet{fruit2018constrained} proved that, similarly to $L$, there exists a solution $(g^+,h^+) \in \Re \times \Re^{S}$ to the optimality equation $\opT{h^+} = h^+ + g^+ e$, and \scopt converges to a solution vector $h^+$ of the optimality equation and $\lim_{n \to +\infty}\opT{}^{n+1}v_0-\opT{}^n v_0 = g^+e$.
Moreover, $g^+ \geq g^*_c$~\citep[][Lem. 8]{fruit2018constrained}.
Finally, under Asm. 6 and 9, the stopping condition of \scopt ensures that $\pi_n$ is an $\varepsilon$-optimal solution of \eqref{eq:opt.superior.spanc} ~\citep[][Thm. 10]{fruit2018constrained}.
 
\subsection{Learning Problem}
Let $M^*$ be the true \emph{unknown} MDP. We consider the learning problem where $\mathcal{S}$, $\mathcal{A}$ and $\rmaxbound$ are \emph{known}, while rewards $r$ and transition probabilities $p$ are \emph{unknown} and need to be estimated on-line. We evaluate the performance of a learning algorithm $\mathfrak{A}$ after $T$ time steps by its cumulative \emph{regret}:
\begin{equation*}\label{eq:regret}
  \Delta(\mathfrak{A},T) = T g^* - \sum_{t=1}^T r_t(s_t,a_t).
\end{equation*}
%
Finally, we assume that the algorithm is provided with the knowledge of a constant $c>0$ such that $\SP{h^*} \leq c$.
This assumption has been widely used in the literature~\citep[see \eg][]{DBLP:journals/mima/Ortner08,DBLP:journals/corr/abs-1302-2550,fruit2018constrained} and, as shown by~\citep{fruit2018truncated}, it is necessary in order to achieve a logarithmic regret bound in weakly-communicating MDPs.




==> backup20180923/symbolsdef.tex <==
% Misc symbols
\newcommand{\M}{\mathcal M}
\newcommand{\A}{\mathcal A}
\renewcommand{\O}{\mathcal O}
\renewcommand{\L}{\mathcal L}
\newcommand{\calS}{\mathcal S}
\newcommand{\calScom}{\mathcal{S}^{\texttt{C}}}
\newcommand{\Scom}{S^{\texttt{C}}}
\newcommand{\calStrans}{\mathcal{S}^{\texttt{T}}}
\newcommand{\Strans}{S^{\texttt{T}}}

\newcommand{\R}{\mathcal R}
\newcommand{\G}{\mathcal G}
\newcommand{\T}{\mathcal T}
\newcommand{\calP}{\mathcal P}
\newcommand{\D}{\mathcal D}
\newcommand{\F}{\mathcal F}
\newcommand{\Prob}{\mathbbm P}
\renewcommand{\Re}{\mathbb R}
\newcommand{\Na}{\mathbb N}
\newcommand{\E}{\mathbb E}
\newcommand{\nextstates}{\Gamma}
\newcommand{\nextstatescom}{\Gamma^{\texttt{C}}}
\newcommand{\diamcom}{D^{\texttt{C}}}
\newcommand{\one}[1]{\mathbbm{1} \left(#1 \right)}
\newcommand{\sigalg}{$\sigma$-algebra\@\xspace}
\newcommand{\sigalgs}{$\sigma$-algebras\@\xspace}
\newcommand{\as}{a.s.\@\xspace}
\newcommand{\rv}{r.v.\@\xspace}
\newcommand{\rvrv}{real-valued r.v.\@\xspace}
\newcommand{\smallplus}{{\scalebox{.5}{+}}}

% Decision rules, policies, constrained sets
\newcommand{\MR}{D^\text{MR}}
\newcommand{\MD}{D^\text{MD}}
\newcommand{\SR}{\Pi^\text{SR}}
\newcommand{\SD}{\Pi^\text{SD}}
\newcommand{\PiC}{\Pi_c}

% operators
\newcommand{\Var}[1]{\mathbb{V}\left({#1}\right)}
\newcommand{\Varcond}[2]{\mathbb{V}\left({#1} \big| {#2}\right)}
\newcommand{\SP}[1]{sp\left\{{#1}\right\}}
\newcommand{\proj}[1]{\Gamma_c{#1}}
\newcommand{\projN}[1]{\Phi{#1}}
\newcommand{\norm}[2][\infty]{\left\|#2\right\|_{#1}}
\DeclareMathOperator*{\argmax}{\arg\,\max}
\DeclareMathOperator*{\argmin}{\arg\,\min}
\DeclareMathOperator*{\arginf}{\arg\,\inf}
\DeclareMathOperator*{\Arg}{Arg}
\DeclareMathOperator*{\Argmax}{\Arg\,\max}
\newcommand{\transpose}[1]{{#1}^\mathsf{T}}
\newcommand{\transp}{\mathsf{T}}
\newcommand{\opT}[1]{T_c#1}
\newcommand{\opN}[1]{N_c{#1}}
\newcommand{\opG}[1]{G_c{#1}}
\newcommand{\lnn}[1]{\ln\left({#1}\right)}
\newcommand{\expp}[1]{\exp\left({#1}\right)}

% names
\newcommand{\regucrl}{{\small\textsc{RegUCRL}}\xspace}
\newcommand{\evi}{{\small\textsc{EVI}}\xspace}
\newcommand{\stevi}{{\small\textsc{STEVI}}\xspace}
\newcommand{\regal}{{\small\textsc{Regal}}\xspace}
\newcommand{\regalc}{{\small\textsc{Regal.C}}\xspace}
\newcommand{\regald}{{\small\textsc{Regal.D}}\xspace}
\newcommand{\scopt}{{\small\textsc{ScOpt}}\xspace}
\newcommand{\ucrl}{{\small\textsc{UCRL}}\xspace}
\newcommand{\uccrl}{{\small\textsc{UCCRL}}\xspace}
\newcommand{\bonusucrl}{{\small\textsc{UCRL}\textsuperscript{+}}\xspace}
\newcommand{\bonusscal}{{\small\textsc{SCAL}\textsuperscript{+}}\xspace}
\newcommand{\psrl}{{\small\textsc{PSRL}}\xspace}
\newcommand{\effpsrl}{{\small\textsc{e-PSRL}}\xspace}
\newcommand{\optpsrl}{{\small\textsc{Opt-PSRL}}\xspace}
\newcommand{\pscal}{{\small\textsc{PSCAL}}\xspace}
\newcommand{\effpscal}{{\small\textsc{e-PSCAL}}\xspace}
\newcommand{\scal}{{\small\textsc{SCAL}}\xspace}
\newcommand{\scalcont}{{\small\textsc{C-SCAL}\textsuperscript{+}}\xspace}
\newcommand{\tucrl}{{\small\textsc{TUCRL}}\xspace}
\newcommand{\ucrlsmdp}{{\small\textsc{UCRL-SMDP}}\xspace}
\newcommand{\sucrl}{{\small\textsc{SUCRL}}\xspace}
\newcommand{\tevi}{{\small\textsc{TEVI}}\xspace}
\newcommand{\freesucrl}{{\small\textsc{FSUCRL}}\xspace}
\newcommand{\freesucrlA}{{\small\textsc{FSUCRLv1}}\xspace}
\newcommand{\freesucrlB}{{\small\textsc{FSUCRLv2}}\xspace}
\newcommand{\pluginsucrl}{{\small\textsc{Est-SUCRL}}\xspace}
%\newcommand{\pluginsucrl}{{\small\textsc{Est-SUCRL}}\xspace}
\newcommand{\rmax}{{\small\textsc{RMax}}\xspace}
\newcommand{\rmaxbound}{r_{\max}}
\newcommand{\rmaxsmdp}{{\small\textsc{RMax-SMDP}}\xspace}
\newcommand{\abs}{\text{abs}}

\newcommand\subsetsim{\mathrel{\substack{
  \textstyle\subset\\[-0.2ex]\textstyle\sim}}}

\newcommand\supsetsim{\mathrel{\substack{
  \textstyle\supset\\[-0.2ex]\textstyle\sim}}}

% short forms 
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wo}[1]{\overline{#1}}
\newcommand{\wb}[1]{\overline{#1}}
\newcommand{\wu}[1]{\underline{#1}}

\usepackage{accents}
\DeclareMathAccent{\wtilde}{\mathord}{largesymbols}{"65}
\newcommand{\uwidetilde}[1]{\underaccent{\wtilde}{#1}}
\newcommand{\uwt}[1]{\underaccent{\wtilde}{#1}}

\newcommand{\pluseq}{\mathrel{+}=}

\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator*{\spn}{sp}
\DeclareMathOperator*{\vect}{Vec}

\DeclareRobustCommand{\eg}{e.g.,\@\xspace}
\DeclareRobustCommand{\ie}{i.e.,\@\xspace}
\DeclareRobustCommand{\aka}{a.k.a.\@\xspace}
\DeclareRobustCommand{\wrt}{w.r.t.\@\xspace}
\DeclareRobustCommand{\wp}{w.p.\@\xspace}
\DeclareRobustCommand{\st}{s.t.\@\xspace}

% % Math environments
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem*{remark}{Remark}

% \theoremstyle{remark}
% \newtheorem*{rem}{Remark}
% \newtheorem*{note}{Note}
% \newtheorem{case}{Case}
% 
% \theoremstyle{theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{conj}{Conjecture}
% \newtheorem{example}{Example}
\newtheorem{assumption}[theorem]{Assumption}

% \renewenvironment{proof}{\fontfamily{cmss}\selectfont \small \textbf{\textit{Proof.}}\vspace{.1cm}}{\hfill$\square$\\ \fontfamily{\familydefault}\selectfont }

%\renewenvironment{example}{\fontfamily{cmss}\selectfont \small \textbf{\textit{Example.}}\vspace{.1cm}}{\hfill$\square$\\ \fontfamily{\familydefault}\selectfont }

% box for algorithms
\newlength{\minipagewidth}
\newlength{\minipagewidthx}
\setlength{\minipagewidth}{0.99\textwidth}
\setlength{\minipagewidthx}{0.99\textwidth}
\setlength{\fboxsep}{1.5mm}
\addtolength{\minipagewidth}{-\fboxrule}
\addtolength{\minipagewidth}{-\fboxrule}
\addtolength{\minipagewidth}{-\fboxsep}
\addtolength{\minipagewidth}{-\fboxsep}
\addtolength{\minipagewidthx}{+\fboxsep}
\newcommand{\bookbox}[1]{
\par\medskip\noindent
\framebox[\columnwidth]{
\begin{minipage}{\minipagewidth} {#1} \end{minipage} } \par\medskip }

\newcommand{\bookboxx}[1]{\small
\par\medskip\noindent
\framebox[0.99\textwidth]{
\begin{minipage}{0.97\dimexpr\textwidth-\parindent\relax} {#1} \end{minipage} } \par\medskip }


==> sec_experiments.tex <==
% !TEX root = main.tex
\section{Experiments}\label{sec:experiments}

For the experiments we consider a tighter concentration inequality for the reward: empirical Bernstein's inequality~\citep{audibert2007tuning,Maurer2009empirical}. This does not affect the regret guarantees but slightly improves the empirical regret at the expense of a negligible additional computational cost. The bonus is then defined using:
\begin{align*}
\beta_{r,k}^{sa}:=
         \sqrt{\frac{14 
                         \wh{\sigma}_{r,k}^2(s,a)
                        b_{k,\delta}
                }{\max\lbrace 1, N_k(s,a)\rbrace}} + \frac{\frac{49}{3}
\rmaxbound
        b_{k,\delta}
        }{\max\lbrace 1, N_k(s,a)-1 \rbrace},\\
\end{align*}
where $\wh{\sigma}_{r,k}^2(s,a)$ is the empirical variance of $r(s,a)$.
Although tighter, this new confidence bound might be of limited practical interest for high dimensional problems as computing $\wh{\sigma}_{r,k}^2(s,a)$ can be computationally expensive.

